Metric-Affine Manifold

We call a manifold with torsion and nonmetricity the metric-affine manifold. The nonmetricity leads to a difference between the auto parallel line and the extreme line, and to a change in the expression of the Frenet transport and moving basis. The torsion leads to a change in the Killing equation. We also need to add a similar equation for the connection. The analysis of the Frenet transport leads to the concept of the Cartan transport and an introduction of the connection compatible with the metric tensor. The dynamics of a particle follows to the Cartan transport. We need additional physical constraints to make a nonmetricity observable.

==> Affine.Russian.tex <==
%auto-ignore
\def\texAffine{}
\ifx\PrintBook\undefined
\else
				\chapter{Геометрия метрико-аффинного многообразия}
\fi

			\section{Кривая экстремальной длины}
			\label{section: Line with extreme length}

Существует два разных определения геодезической в римановом многообразии.
Одно из них опирается на параллельный перенос.
Мы будем называть соответствующую
\AddIndex{кривую автопараллельной}{auto parallel line}.
Другое определение опирается на длину траектории.
Мы будем называть соответствующую
\AddIndex{кривую экстремальной}{extreme line}.
В метрико\hyph аффинном многообразие эти линии имеют различные
уравнения \citeBib{torsion}.
Уравнение автопараллельной кривой не меняе. Однако, уравнение
экстремальной кривой меняется\footnote{Чтобы вывести
уравнение \eqref{eq: xtremeLine},
я следую идеям, которые Рашевский \citeBib{Rashevsky}
использовал для Риманова многообразия}.

		\begin{theorem}
Пусть $x^i = x^i(t,\alpha)$ - кривая, зависящая от параметра $\alpha$,
с фиксированными точками при $t = t_1$ и
$t = t_2$, и мы определяем её длину как
\begin{equation}
s = \int^{t_2}_{t_1} \sqrt{g_{ij} \frac {dx^i} {dt} \frac {dx^j} {dt}} dt
\label{eq: LineLength}
\end{equation}
Тогда 
%\begin{widetext}
\begin{equation}
\delta s =
\int^{t_2}_{t_1} \left( \frac 1 2 \left(
g_{kj;i}- g_{ik;j}
- g_{ij;k} \right) \frac{dx^k}{ds} \frac{dx^j}{ds} ds -
g_{ij} D\frac {dx^j} {ds} \right) \delta x^i
\label{eq: VarLineLength}
\end{equation}
%\end{widetext}
где $\delta x^k$ - изменение длины, когда $\alpha$ меняется.
		\end{theorem}
		\begin{proof}
Имеем
$$\frac {ds} {dt} = \sqrt{g_{ij} \frac {dx^i} {dt} \frac {dx^j} {dt}}$$
и
\[
\delta s = \int^{t_2}_{t_1}
\frac
 {\delta \left( g_{ij} \frac{dx^i}{dt} \frac{dx^j}{dt} \right)}
 {2 \frac{ds}{dt}} dt
\]

Мы можем оценить знаменатель этой дроби
\[
g_{ij,k} \delta x^k \frac {dx^i} {dt} \frac {dx^j} {dt} +
2 g_{ij} \delta \frac {dx^i} {dt} \frac {dx^j} {dt} =
\]
%\begin{widetext}
\[
= g_{ij;k} \delta x^k {dx^i} {dt} \frac {dx^j} {dt} +
2 g_{ij} \Gamma^i_{lk} \delta x^k \frac {dx^l} {dt} \frac {dx^j} {dt}
+2 g_{ij} d \frac {\delta x^i} {dt} \frac {dx^j} {dt} =
\]
%\end{widetext}
\[
= g_{ij;k} \delta x^k \frac{dx^i}{dt} \frac{dx^j}{dt} + 2 g_{ij} \frac{D\delta x^i}{dt} \frac{dx^j}{dt}
\]
и мы имеем
\[
\delta s = \int^{t_2}_{t_1}
{
 \frac
 {
  g_{ij;k} \delta x^k dx^i \frac{dx^j}{dt} + 2 g_{ij} D\delta x^i \frac{dx^j}{dt}
 } 
 {2 \frac {ds} {dt}}
}
\]
\[
= \int^{t_2}_{t_1}
\left(\frac 1 2 g_{ij;k} \delta x^k dx^i \frac {dx^j} {ds} +
g_{ij} D\delta x^i \frac {dx^j} {ds} \right) 
\]
%\begin{widetext}
\[
= \int^{t_2}_{t_1}
\left(\frac 1 2 g_{kj;i} \delta x^i \frac {dx^k} {ds} {ds} \frac {dx^j} {ds} +
d\left(g_{ij} \delta x^i \frac {dx^j} {ds}\right)
-g_{ij;k} \frac {dx^k} {ds} {ds} \frac {dx^j} {ds} \delta x^i -
g_{ij} D\frac {dx^j} {ds} \delta x^i\right) \]
\[
= 
\left.\left(g_{ij} \delta x^i \frac{dx^j}{ds} \right)\right|^{t_2}_{t_1}
+ \int^{t_2}_{t_1} \left(\frac 1 2 \left(
g_{kj;i} -
g_{ij;k} -
g_{ik;j} \right) \frac {dx^k} {ds} \frac{dx^j}{ds} {ds}
- g_{ij} D\frac{dx^j}{ds}\right) \delta x^i
\]
%\end{widetext}
Первое слагаемое равно $0$, так как точки, где $t = t_1$ и $t = t_2$, зафиксированы.
Следовательно, мы доказали утверждение теоремы.
		\end{proof}

		\begin{theorem}
		\label{theorem: xtremeLine}
Экстремальная кривая удовлетворяет уравнению
	\begin{equation}
\label{eq: xtremeLine}
\frac {D\frac {dx^l} {ds}} {ds} =
\frac 1 2 g^{il} \left(g_{kj;i} - g_{ik;j}
- g_{ij;k}\right) \frac{dx^k}{ds} \frac{dx^j}{ds}
	\end{equation}
		\end{theorem}
		\begin{proof}
Чтобы найти линию экстремальной длины,
мы воспользуемся функционалом \eqref{eq: LineLength}.
Так как $\delta s = 0$, то
$$
\frac 1 2 \left(g_{kj;i} -
g_{ij;k} -
g_{ik;j}\right) \frac {dx^k} {ds} \frac {dx^j} {ds} ds
- g_{ij} D\frac {dx^j} {ds} = 0$$
следует из \eqref{eq: VarLineLength}.
		\end{proof}

		\begin{theorem}
Параллельный перенос вдоль экстремальной кривой
сохраняет длину касательного вектора.
		\end{theorem}

		\begin{proof}

Пусть $$v^i=\frac {dx^i}{ds}$$ - касательный вектор к экстремальной кривой.
Из теоремы \ref{theorem: xtremeLine} следует, что
$$\frac {Dv^l} {ds} =
g^{il} \frac 1 2 \left(g_{kj;i} - g_{ik;j}
- g_{ij;k}\right) v^k v^j
$$
и
$$\frac {Dg_{kl} v^k v^l}{ds}
= \frac {Dg_{kl}} {ds}v^k v^l
+ g_{kl}\frac {Dv^k} {ds} v^l
+ g_{kl}v^k \frac {Dv^l} {ds}=$$
$$= g_{kl;p}v^p v^k v^l+$$
$$+ g_{kl}g^{ik} \frac 1 2 \left(g_{rj;i} - g_{ir;j}
- g_{ij;r}\right) v^r v^j v^l
+ g_{kl}v^k g^{il} \frac 1 2 \left(g_{rj;i} - g_{ir;j}
- g_{ij;r}\right) v^r v^j=$$
$$= g_{kl;p}v^p v^k v^l
+ \left(g_{rj;l} - g_{lr;j}
- g_{lj;r}\right) v^r v^j v^l = 0$$
Следовательно длина вектора $v^i$ не меняется вдоль экстремальной кривой.
		\end{proof}

			\section{Перенос Френе}
			\label{section: Frenet Transport}

Все уравнения, которые мы выводили до сих пор, различны,
однако они имеют нечто общее в своей структуре.
Все эти уравнения выражают движение вдоль кривой и в их правой части
мы можем видеть кривизну этой кривой.

По определению, кривизна кривой равна
\[\xi(s) = \left| \frac {D\frac {dx^l} {ds}} {ds} \right|\]
Следовательно, мы можем определить единичный вектор $e_1$ такой, что
\[\frac {D\frac {dx^l} {ds}} {ds} = \xi e^l_1\]

Знание переноса базиса вдоль кривой очень важно,
так как это позволяет нам изучать как изменяется пространство время,
когда наблюдатель совершает движение.
Наша задача - найти уравнения, подобные переносу Френе в
римановом пространстве. Мы строим сопутствующий базис $\nu^i_k$ таким же
образом, как мы это делаем в римановом пространстве.

Векторы
\[\xi^i(t)=\frac{dx^i(t)}{dt}, \ \ \ \frac {D\xi^i} {dt},
\ \ \ ...\ \ \ \frac {D^{n-1}\xi^i} {dt^{n-1}}\]
вообще говоря, линейно независимы. Мы называем плоскость, построенную
на базе первых $p$ векторов, $p$-ой соприкасающейся плоскостью $R_p$.
Эта плоскость не зависит от выбора параметра $t$.

Наша следующая задача - построить ортогональный базис, который
покажет нам, как кривая изменяется.
Мы берём вектор $\nu^i_1\in R_1$ так, что он касателен к кривой.
Мы берём вектор $\nu^i_p\in R_p$, $p>1$ так, что $\nu^i_p$
ортогонален $R_{p-1}$. Если исходная кривая не изотропна,
то каждый $\nu^i_p$ также не изотропен и мы можем взять единичный вектор
в том же направлении. Мы называем этот базис сопутствующим.

		\begin{theorem}
		\label{theorem: FrenetTransfer}
\AddIndex{Перенос Френе}{Frenet transport} в метрико-аффинном многообразии имеет вид
	\begin{equation}
	\begin{split}
\frac {D\nu^i_p} {dt}
= \frac 1 2 g^{im}(g_{kl;m}-g_{km;l}-g_{ml;k}) \nu^k_1 \nu^l_p - \\
- \epsilon_p \epsilon_{p-1} \xi_{p-1} \nu^i_{p-1} + \xi_p \nu^i_{p+1}
	\end{split}
	\label{eq: Frenet}
	\end{equation}
\[\epsilon_k = sign(g_{pq} \nu^p_k \nu^q_k)\]
Здесь $\nu^a_k$ - вектор базиса, движущегося вдоль кривой,
\[\epsilon_k = sign(g_{pq} \nu^p_k \nu^q_k)\]
		\end{theorem}
		\begin{proof}
Мы определяем векторы $\nu^a_k$ таким образом, что
	\begin{equation}
\frac {D\nu^i_p} {dt}
= \frac 1 2 g^{im}(g_{kl;m}-g_{km;l}-g_{ml;k}) \nu^k_1 \nu^l_p
+ a^q_p \nu^i_q
	\label{eq: Frenet_1}
	\end{equation}
где $a_p^q = 0$, когда $q > p+1$.
Теперь мы можем определить коэффициенты $a^q_p$. Если мы возьмём
производную уравнения
\[
g_{ij} \nu^i_p \nu^j_p = const
\]
и подставим \eqref{eq: Frenet_1}, мы получим уравнение
\[\frac {dg_{ij}\nu^i_a \nu^j_b} {ds}=
\frac {Dg_{ij}} {ds}\nu^i_a \nu^j_b+
g_{ij}\frac {D\nu^i_a} {ds}\nu^j_b+
g_{ij}\nu^i_a\frac {D\nu^j_b} {ds}=\]
\[=g_{ij;k}\nu^k_1 \nu^i_a \nu^j_b+\]
\[+g_{ij}(\frac 1 2 g^{im}(g_{kl;m}-g_{km;l}-g_{ml;k}) \nu^k_1 \nu^l_a
+ a^q_a \nu^i_q)\nu^j_b+\]
\[+g_{ij}\nu^i_a (\frac 1 2 g^{jm}(g_{kl;m}-g_{km;l}-g_{ml;k}) \nu^k_1 \nu^l_b
+ a^q_b \nu^i_q)=\]
\[=g_{ij;k}\nu^k_1 \nu^i_a \nu^j_b+\]
\[+g_{ij}\frac 1 2 g^{im}(g_{kl;m}-g_{km;l}-g_{ml;k}) \nu^k_1 \nu^l_a\nu^j_b
+ g_{ij}a^q_a \nu^i_q\nu^j_b+\]
\[+g_{ij}\nu^i_a \frac 1 2 g^{jm}(g_{kl;m}-g_{km;l}-g_{ml;k}) \nu^k_1 \nu^l_b
+ g_{ij}\nu^i_a a^q_b \nu^i_q=\]
\[=\frac 1 2 \nu^k_1 \nu^i_a \nu^j_b(2g_{ij;k}+
g_{ki;j}-g_{kj;i}-g_{ji;k}+
g_{kj;i}-g_{ki;j}-g_{ij;k})+\]
\[+ \epsilon_b a^b_a+
+ \epsilon_a a^a_b=0\]

$a_p^q = 0$, когда $q > p+1$ по определению.
Следовательно $a_p^q = 0$, когда $q < p+1$.
Полагая $\xi_p = a^{p+1}_p$, мы получим
\[
a^p_{p+1} = - \epsilon_p \epsilon_{p+1} \xi_p 
\]
Когда $q = p$, мы получим
\[
a_{p,p} = 0
\]
Мы получим \eqref{eq: Frenet}, когда подставим $a^q_p$ в \eqref{eq: Frenet_1}.
		\end{proof}

			\section{Производная Ли}
			\label{section: Lie Derivative}

Векторное поле $\xi^k$ на многообразии порождает инфинитезимальное преобразование
	\begin{equation}
	\label{eq: infinitesimal displacement}
x'^k=x^k+\epsilon\xi^k
	\end{equation}
которое ведёт к \AddIndex{производной Ли}{Lie derivative}.
Производная Ли говорит нам, как объект изменяется,
когда мы движемся вдоль векторного поля.

		\begin{theorem}
\AddIndex{Производная Ли метрики}{Lie derivative of metric} имеет вид
\symb{\mathcal{L}_\xi g_{ab}}0{Lie derivative of metric}
	\begin{equation}
	\label{eq: Lie derivative of metric}
\ShowSymbol{Lie derivative of metric}=\xi^k_{;<a>}g_{kb}+\xi^k_{;<b>}g_{ka}
+T^l_{ka}g_{lb}\xi^k+T^l_{kb}g_{la}\xi^k+g_{ab;<k>}\xi^k
	\end{equation}
		\end{theorem}
		\begin{proof}
Мы начнём с преобразования \eqref{eq: infinitesimal displacement}.
Тогда
\[g_{ab}(x')=g_{ab}(x)+g_{ab,c}\epsilon \xi^c\]
	\begin{align*}
g'_{ab}(x')&=\frac{\partial x^c}{\partial x'^a} \frac{\partial x^d}{\partial x'^b}g_{cd}(x)\\
&=g_{ab}-\epsilon \xi^c_{,a}g_{cb}-\epsilon \xi^c_{,b}g_{ac}
	\end{align*}
Согласно определению производной Ли, мы имеем
	\begin{align*}
\mathcal{L}_\xi g_{ab}&=g_{ab}(x')-g'_{ab}(x')\\
&=g_{ab,c}\epsilon \xi^c+\epsilon \xi^c_{,a}g_{cb}+\epsilon \xi^c_{,b}g_{ac}\\
&=(g_{ab;<c>}+\overline{\Gamma^d_{ac}}g_{db}+\overline{\Gamma^d_{bc}}g_{ad})\epsilon \xi^c\\
&+\epsilon (\xi^c_{;<a>}-\overline{\Gamma^c_{da}}\xi^d)g_{cb}
+\epsilon (\xi^c_{;<b>}-\overline{\Gamma^c_{db}}\xi^d)g_{ac}
	\end{align*}
	\begin{equation}
	\begin{split}
\mathcal{L}_\xi g_{ab}&=g_{ab;<c>} \xi^c+\overline{\Gamma^d_{ac}}g_{db} \xi^c+\overline{\Gamma^d_{bc}}g_{ad}\xi^c\\
&+ \xi^c_{;<a>}g_{cb}- \overline{\Gamma^c_{da}}\xi^dg_{cb}
+ \xi^c_{;<b>}g_{ac}- \overline{\Gamma^c_{db}}\xi^dg_{ac}
	\end{split}
	\label{eq: Lie derivative of metric,1}
	\end{equation}
\eqref{eq: Lie derivative of metric} следует из
\eqref{eq: Lie derivative of metric,1} и \eqref{eq: Torsion coordinates}.
		\end{proof}
		\begin{theorem}
\AddIndex{Производная Ли связности}{Lie derivative of connection} имеет вид
\symb{\mathcal{L}_\xi\Gamma^a_{bc}}0{Lie derivative of connection}
	\begin{equation}
	\label{eq: Lie derivative of connection}
\ShowSymbol{Lie derivative of connection}=-\overline{R^a_{bcp}}\xi^p
-T^a_{bp;<c>}\xi^p
-T^a_{be}\xi^e_{;<c>}
+\xi^a_{;<bc>}
	\end{equation}
		\end{theorem}
		\begin{proof}
Мы начнём с преобразования \eqref{eq: infinitesimal displacement}.
Тогда
	\begin{equation}
	\begin{split}
\overline{\Gamma^a_{bc}(x')}
&=\Gamma^a_{bc}(x')+A^a_{bc}(x')\\
&=\Gamma^a_{bc}(x)+\Gamma^a_{bc,p}\epsilon \xi^p+A^a_{bc}(x)+A^a_{bc,p}\epsilon \xi^p\\
&=\overline{\Gamma^a_{bc}(x)}+\overline{\Gamma^a_{bc,p}}\epsilon \xi^p
	\end{split}
	\label{eq: Lie derivative of connection,1}
	\end{equation}
	\begin{align*}
\overline{\Gamma'^a_{bc}}(x')
&=\Gamma'^a_{bc}(x')+A'^a_{bc}(x')\\
&=\frac{\partial x'^a}{\partial x^e}\frac{\partial x^f}{\partial x'^b} \frac{\partial x^g}{\partial x'^c}
\Gamma^e_{fg}(x)
+\frac{\partial x'^a}{\partial x^e}\frac{\partial^2 x^e}{\partial x'^b\partial x'^c}
+\frac{\partial x'^a}{\partial x^e}\frac{\partial x^f}{\partial x'^b} \frac{\partial x^g}{\partial x'^c}
A^e_{fg}(x)\\
&=\Gamma^a_{bc}+\epsilon \xi^a_{,e}\Gamma^e_{bc}
-\epsilon \xi^e_{,b}\Gamma^a_{ec}-\epsilon \xi^e_{,c}\Gamma^a_{be}
+(\delta^a_e+\epsilon \xi^a_{,e})(-\epsilon \xi^e_{,cb}))\\
&+A^a_{bc}+\epsilon \xi^a_{,e}A^e_{bc}
-\epsilon \xi^e_{,b}A^a_{ec}-\epsilon \xi^e_{,c}A^a_{be}
	\end{align*}
	\begin{equation}
\overline{\Gamma'^a_{bc}}(x')
=\overline{\Gamma^a_{bc}}+\epsilon \xi^a_{,e}\overline{\Gamma^e_{bc}}
-\epsilon \xi^e_{,b}\overline{\Gamma^a_{ec}}-\epsilon \xi^e_{,c}\overline{\Gamma^a_{be}}
-\epsilon \xi^a_{,cb}
	\label{eq: Lie derivative of connection,2}
	\end{equation}
По определению
\[
\xi^a_{;<e>}
=\xi^a_{,e}
+\overline{\Gamma^a_{pe}} \xi^p
\]
	\begin{equation}
\xi^a_{,e}
=\xi^a_{;<e>}
-\overline{\Gamma^a_{pe}} \xi^p
	\label{eq: Lie derivative of connection,3}
	\end{equation}
	\begin{align*}
\xi^a_{;<ef>}
&=\xi^a_{;<e>,f}
+\overline{\Gamma^a_{pf}} \xi^p_{;<e>}
-\overline{\Gamma^p_{ef}} \xi^a_{;<p>}\\
&=\xi^a_{,ef}+\overline{\Gamma^a_{pe,f}} \xi^p+\overline{\Gamma^a_{pe}} \xi^p_{,f}
+\overline{\Gamma^a_{pf}} \xi^p_{;<e>}
-\overline{\Gamma^p_{ef}} \xi^a_{;<p>}\\
&=\xi^a_{,ef}+\overline{\Gamma^a_{pe,f}} \xi^p
+\overline{\Gamma^a_{pe}} \xi^p_{;<f>}-\overline{\Gamma^a_{pe}} \overline{\Gamma^p_{rf}} \xi^r
+\overline{\Gamma^a_{pf}} \xi^p_{;<e>}
-\overline{\Gamma^p_{ef}} \xi^a_{;<p>}
	\end{align*}
	\begin{equation}
\xi^a_{,ef}
=\xi^a_{;<ef>}-\overline{\Gamma^a_{pe,f}} \xi^p
-\overline{\Gamma^a_{pe}} \xi^p_{;<f>}+\overline{\Gamma^a_{pe}} \overline{\Gamma^p_{rf}} \xi^r
-\overline{\Gamma^a_{pf}} \xi^p_{;<e>}
+\overline{\Gamma^p_{ef}} \xi^a_{;<p>}
	\label{eq: Lie derivative of connection,4}
	\end{equation}
Мы подставим \eqref{eq: Lie derivative of connection,4} и \eqref{eq: Lie derivative of connection,3}
в \eqref{eq: Lie derivative of connection,2} и получим
	\begin{align*}
&\overline{\Gamma'^a_{bc}}(x')\\
&=\overline{\Gamma^a_{bc}}+\epsilon (\underline{\xi^a_{;<e>}}_{4:T}
-\overline{\Gamma^a_{pe}} \xi^p)\overline{\Gamma^e_{bc}}
-\epsilon (\underline{\xi^e_{;<b>}}_2
-\underline{\overline{\Gamma^e_{pb}} \xi^p}_1)\overline{\Gamma^a_{ec}}-\epsilon (\underline{\xi^e_{;<c>}}_{3:T}
-\overline{\Gamma^e_{pc}} \xi^p)\overline{\Gamma^a_{be}}\\
&-\epsilon (\xi^a_{;<cb>}-\overline{\Gamma^a_{pc,b}} \xi^p
-\underline{\overline{\Gamma^a_{pc}} \xi^p_{;<b>}}_2
+\underline{\overline{\Gamma^a_{pc}} \overline{\Gamma^p_{rb}} \xi^r}_1
-\underline{\overline{\Gamma^a_{pb}} \xi^p_{;<c>}}_3
+\underline{\overline{\Gamma^p_{cb}} \xi^a_{;<p>}}_4)
	\end{align*}
	\begin{equation}
\overline{\Gamma'^a_{bc}}(x')
=\overline{\Gamma^a_{bc}}+\epsilon (\xi^a_{;<e>}T^e_{cb}
-\overline{\Gamma^a_{pe}} \xi^p\overline{\Gamma^e_{bc}}
+\xi^e_{;<c>}T^a_{be}
+\overline{\Gamma^e_{pc}} \xi^p\overline{\Gamma^a_{be}}
-\xi^a_{;<cb>}+\overline{\Gamma^a_{pc,b}} \xi^p)
	\label{eq: Lie derivative of connection,5}
	\end{equation}
Согласно определению производной Ли, мы имеем,
пользуясь \eqref{eq: Lie derivative of connection,1} и \eqref{eq: Lie derivative of connection,5},
	\begin{align*}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}
&=(\overline{\Gamma^a_{bc}}(x')-\overline{\Gamma'^a_{bc}}(x'))\epsilon^{-1}\\
&=(\overline{\Gamma^a_{bc}}+\overline{\Gamma^a_{bc,p}}\epsilon \xi^p\\
&-\overline{\Gamma^a_{bc}}-\epsilon (\xi^a_{;<e>}T^e_{cb}
-\overline{\Gamma^a_{pe}} \xi^p\overline{\Gamma^e_{bc}}
+\xi^e_{;<c>}T^a_{be}
+\overline{\Gamma^e_{pc}} \xi^p\overline{\Gamma^a_{be}}
-\xi^a_{;<cb>}+\overline{\Gamma^a_{pc,b}} \xi^p))\epsilon^{-1}
	\end{align*}
	\begin{equation}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}=\overline{\Gamma^a_{bc,p}} \xi^p
-\xi^a_{;<e>}T^e_{cb}
+\overline{\Gamma^a_{pe}} \xi^p\overline{\Gamma^e_{bc}}
-\xi^e_{;<c>}T^a_{be}
-\overline{\Gamma^e_{pc}} \xi^p\overline{\Gamma^a_{be}}
+\xi^a_{;<cb>}-\overline{\Gamma^a_{pc,b}} \xi^p
	\label{eq: Lie derivative of connection,6}
	\end{equation}
Из \eqref{eq: Lie derivative of connection,6}
и \eqref{eq: Torsion coordinates} следует, что
	\begin{align*}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}
&=\overline{\Gamma^a_{cb,p}} \xi^p-\overline{\Gamma^a_{cp,b}} \xi^p\\
&+\underline{\overline{\Gamma^a_{pe}} \overline{\Gamma^e_{bc}}\xi^p}_{3:T}
-\underline{\overline{\Gamma^a_{ep}} \overline{\Gamma^e_{bc}}\xi^p}_3
+\underline{\overline{\Gamma^a_{ep}} \overline{\Gamma^e_{bc}}\xi^p}_{4:T}
-\underline{\overline{\Gamma^a_{ep}} \overline{\Gamma^e_{cb}}\xi^p}_4
+\overline{\Gamma^a_{ep}} \overline{\Gamma^e_{cb}}\xi^p\\
&-\underline{\overline{\Gamma^e_{pc}} \overline{\Gamma^a_{be}}\xi^p}_{1:T}
+\underline{\overline{\Gamma^e_{pc}} \overline{\Gamma^a_{eb}}\xi^p}_1
- \underline{\overline{\Gamma^a_{eb}}\overline{\Gamma^e_{pc}}\xi^p}_{2:T}
+\underline{\overline{\Gamma^a_{eb}}\overline{\Gamma^e_{cp}}\xi^p}_2
-\overline{\Gamma^a_{eb}}\overline{\Gamma^e_{cp}}\xi^p\\
& -\xi^a_{;<e>}T^e_{cb}
-\xi^e_{;<c>}T^a_{be}
+\xi^a_{;<cb>}-T^a_{cp,b} \xi^p-T^a_{bc,p} \xi^p
	\end{align*}
	\begin{equation}
	\begin{split}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}
&=\overline{\Gamma^a_{cb,p}} \xi^p-\overline{\Gamma^a_{cp,b}} \xi^p
+\overline{\Gamma^a_{ep}} \overline{\Gamma^e_{cb}}\xi^p
-\overline{\Gamma^a_{eb}}\overline{\Gamma^e_{cp}}\xi^p\\
&-\underline{T^a_{pe} \overline{\Gamma^e_{bc}}\xi^p}_{4:T}-\underline{\overline{\Gamma^a_{ep}} T^e_{bc}\xi^p}_1
-\underline{\overline{\Gamma^e_{pc}} T^a_{eb}\xi^p}_{3:T}- \underline{\overline{\Gamma^a_{eb}}T^e_{cp}\xi^p}_2\\
& -\xi^a_{;<e>}T^e_{cb}
-\xi^e_{;<c>}T^a_{be}+\xi^a_{;<cb>}\\
&-T^a_{cp;<b>} \xi^p
+\underline{\overline{\Gamma^a_{eb}} T^e_{cp}\xi^p}_2
-\underline{\overline{\Gamma^e_{cb}} T^a_{ep}\xi^p}_4
-\underline{\overline{\Gamma^e_{pb}} T^a_{ce}\xi^p}_{5:T}\\
&-T^a_{bc;<p>} \xi^p
+\underline{\overline{\Gamma^a_{ep}} T^e_{bc}\xi^p}_1-\underline{\overline{\Gamma^e_{bp}} T^a_{ec}\xi^p}_5
-\underline{\overline{\Gamma^e_{cp}} T^a_{be}\xi^p}_3
	\end{split}
	\label{eq: Lie derivative of connection,7}
	\end{equation}
из \eqref{eq: Lie derivative of connection,7} и \xEqRef{0405.027}{eq: GLn curvature} следует, что
	\[
	\begin{split}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}&=\overline{R^a_{cpb}} \xi^p\\
&-T^e_{cp} T^a_{eb}\xi^p
-T^a_{pe} T^e_{cb}\xi^p-T^e_{bp} T^a_{ce}\xi^p\\
& -\xi^a_{;<e>}T^e_{cb}
-\xi^e_{;<c>}T^a_{be}+\xi^a_{;<cb>}\\
&-T^a_{cp;<b>} \xi^p
-T^a_{bc;<p>} \xi^p
	\end{split}
	\]
	\begin{equation}
	\label{eq: Lie derivative of connection,8}
	\begin{split}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}&=-\overline{R^a_{cbp}} \xi^p\\
&- (T^a_{eb}T^e_{cp}
+T^a_{ep} T^e_{bc}+ T^a_{ec}T^e_{pb})\xi^p\\
& -\xi^a_{;<e>}T^e_{cb}
-\xi^e_{;<c>}T^a_{be}+\xi^a_{;<cb>}\\
&-T^a_{cp;<b>} \xi^p
-T^a_{bc;<p>} \xi^p
	\end{split}
	\end{equation}
из \eqref{eq: Lie derivative of connection,8} и \eqref{eq: Bianchi 1} следует, что
	\[
	\begin{split}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}&=\underline{\overline{R^a_{cpb}} \xi^p}_1\\
&- \overline{R^a_{bcp}}\xi^p
-\overline{R^a_{pbc}}\xi^p- \underline{\overline{R^a_{cpb}}\xi^p}_1\\
&+\underline{T^a_{bc:<p>}\xi^p}_3
+T^a_{pb;<c>}\xi^p+ \underline{T^a_{cp;<b>}\xi^p}_2\\
& -\xi^a_{;<e>}T^e_{cb}
-\xi^e_{;<c>}T^a_{be}+\xi^a_{;<cb>}\\
&-\underline{T^a_{cp;<b>} \xi^p}_2
-\underline{T^a_{bc;<p>} \xi^p}_3
	\end{split}
	\]
	\begin{equation}
	\label{eq: Lie derivative of connection,9}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}=-\overline{R^a_{bcp}}\xi^p
-\overline{R^a_{pbc}}\xi^p
-T^a_{bp;<c>}\xi^p
-\xi^a_{;<e>}T^e_{cb}
-\xi^e_{;<c>}T^a_{be}+\xi^a_{;<cb>}
	\end{equation}
Мы подставим \eqref{eq: commutator second derivative of vector} в \eqref{eq: Lie derivative of connection,9}
	\begin{equation}
	\label{eq: Lie derivative of connection,10}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}=-\overline{R^a_{bcp}}\xi^p
-T^a_{bp;<c>}\xi^p
-\underline{T^e_{cb}\xi^a_{;<e>}}_1
-T^a_{be}\xi^e_{;<c>}
-\underline{T^p_{bc}\xi^a_{;<p>}}_1+\xi^a_{;<bc>}
	\end{equation}
\eqref{eq: Lie derivative of connection} следует из \eqref{eq: Lie derivative of connection,10}.
		\end{proof}
		\begin{corollary}
Производная Ли связности в римановом пространстве имеет вид
	\begin{equation}
	\label{eq: Lie derivative of connection in Rieman space}
\mathcal{L}_\xi\Gamma^a_{bc}=-R^a_{cbp} \xi^p+\xi^a_{;cb}\\
	\end{equation}
		\end{corollary}
		\begin{proof}
\eqref{eq: Lie derivative of connection in Rieman space} следует
из \eqref{eq: Lie derivative of connection}, когда $T^a_{bc}=0$
		\end{proof}

			\section{Тождество Бианки}
			\label{section: Bianchi Identity}

		\begin{theorem}
 Первое тождество Бианки для пространства с кручением имеет вид
	\begin{equation}
	\label{eq: Bianchi 1}
	\begin{split}
&T^k_{ij;<m>}+T^k_{mi;<j>}+T^k_{jm;<i>}
+ T^k_{pi}T^p_{jm}+ T^k_{pm}T^p_{ij}+ T^k_{pj}T^p_{mi}\\
&=\overline{R^k_{jmi}}+\overline{R^k_{ijm}}+\overline{R^k_{mij}}
	\end{split}
	\end{equation}
		\end{theorem}
		\begin{proof}
Дифференциал равенства \eqref{eq: Torsion 1} имеет вид
\[
T^k_{ij,m}\theta^m\wedge\theta^i\wedge\theta^j
=(\overline{\Gamma^k_{ji,m}}-\overline{\Gamma^k_{ij,m}})\theta^m\wedge\theta^i\wedge\theta^j
\]
Две формы равны, когда их коэффициенты равны. Следовательно
\[
T^k_{ij,m}+T^k_{mi,j}+T^k_{jm,i}
=\overline{\Gamma^k_{ji,m}}-\overline{\Gamma^k_{ij,m}}
+\overline{\Gamma^k_{im,j}}-\overline{\Gamma^k_{mi,j}}
+\overline{\Gamma^k_{mj,i}}-\overline{\Gamma^k_{jm,i}}
\]
Мы выразим производные, пользуясь ковариантными производными,
и изменим порядок слагаемых
	\begin{align*}
&T^k_{ij;<m>}-\underline{\overline{\Gamma^k_{pm}} T^p_{ij}}_4
+\underline{\overline{\Gamma^p_{im}} T^k_{pj}}_{2:T}-\underline{\overline{\Gamma^p_{jm}} T^k_{pi}}_{3:T}\\
&+T^k_{mi;<j>}-\underline{\overline{\Gamma^k_{pj}} T^p_{mi}}_5
+\underline{\overline{\Gamma^p_{mj}} T^k_{pi}}_3-\underline{\overline{\Gamma^p_{ij}} T^k_{pm}}_{1:T}\\
&+T^k_{jm;<i>}-\underline{\overline{\Gamma^k_{pi}} T^p_{jm}}_6
+\underline{\overline{\Gamma^p_{ji}} T^k_{pm}}_1-\underline{\overline{\Gamma^p_{mi}} T^k_{pj}}_2\\
&=\overline{\Gamma^k_{ji,m}}-\overline{\Gamma^k_{jm,i}}
+\overline{\Gamma^k_{pm}} \overline{\Gamma^p_{ji}}
-\overline{\Gamma^k_{pi}} \overline{\Gamma^p_{jm}}
-\underline{\overline{\Gamma^k_{pm}} \overline{\Gamma^p_{ji}}}_4
+\underline{\overline{\Gamma^k_{pi}} \overline{\Gamma^p_{jm}}}_6\\
&+\overline{\Gamma^k_{im,j}}-\overline{\Gamma^k_{ij,m}}
+\overline{\Gamma^k_{pj}} \overline{\Gamma^p_{im}}
-\overline{\Gamma^k_{pm}} \overline{\Gamma^p_{ij}}
-\underline{\overline{\Gamma^k_{pj}} \overline{\Gamma^p_{im}}}_5
+\underline{\overline{\Gamma^k_{pm}} \overline{\Gamma^p_{ij}}}_4\\
&+\overline{\Gamma^k_{mj,i}}-\overline{\Gamma^k_{mi,j}}
+\overline{\Gamma^k_{pi}} \overline{\Gamma^p_{mj}}-\overline{\Gamma^k_{pj}} \overline{\Gamma^p_{mi}}
-\underline{\overline{\Gamma^k_{pi}} \overline{\Gamma^p_{mj}}}_6
+\underline{\overline{\Gamma^k_{pj}} \overline{\Gamma^p_{mi}}}_5
	\end{align*}
	\begin{equation}
	\label{eq: Bianchi 1,1}
	\begin{split}
&T^k_{ij;<m>}
+T^p_{mi} T^k_{pj}+T^p_{jm} T^k_{pi}
+T^k_{mi;<j>}
+T^p_{ij} T^k_{pm}
+T^k_{jm;<i>}\\
&=\overline{R^k_{jmi}}
+\overline{R^k_{ijm}}
+\overline{R^k_{mij}}
	\end{split}
	\end{equation}
\eqref{eq: Bianchi 1} следует из \eqref{eq: Bianchi 1,1}.
		\end{proof}

%If мы получим derivative of form (\ref{eq: Torsion})
%мы will получим first Bianchi identity for space with кручение \citeBib{Neeman}
%\[D T^a = \Omega^a_c \wedge \theta^c\]
%из \eqref{eq: Torsion} и \eqref{eq: Bianchi 1,1}

Если мы возьмём производную формы \xEqRef{0405.027}{eq: Curvature},
мы увидим, что второе тождество Бианки не
зависит от кручения. 

			\section{Вектор Килинга}
			\label{section: Killing Vector}

Инвариантность метрического тензора $g$ при инфинитезимальном координатном преобразовании
\eqref{eq: infinitesimal displacement}
приводит к \AddIndex{уравнению Килинга}{Killing equation}.

		\begin{theorem}
Уравнение Килинга в метрико\hyph аффинном многообразии имеет вид
	\begin{equation}
	\label{eq: Killing equation 1}
\xi^k_{;<a>}g_{kb}+\xi^k_{;<b>}g_{ka}+T^l_{ka}g_{lb}\xi^k+T^l_{kb}g_{la}\xi^k+g_{ab;<k>}\xi^k=0
	\end{equation}
		\end{theorem}
		\begin{proof}
Инвариантность метрического тензора $g$ означает, что его производная Ли равна $0$
	\begin{equation}
\mathcal{L}_\xi g_{ab}=0
	\label{eq: Killing equation 1,1}
	\end{equation}
\eqref{eq: Killing equation 1} folows из \eqref{eq: Killing equation 1,1} и \eqref{eq: Lie derivative of metric}.
		\end{proof}

%However it looks like for the metric\hyph affine manifold the Killing equation is not
%a sufficient condition for homogeneity of event space. Мы need to write a similar condition
%for the connection as well.

		\begin{theorem}
Условие инвариантности связности в метрико\hyph аффинном многообразии имеет вид
	\begin{equation}
	\label{eq: Killing equation 2}
	\begin{split}
\xi^a_{;<bc>}=\overline{R^a_{bcp}}\xi^p
+T^a_{bp;<c>}\xi^p
+T^a_{bp}\xi^p_{;<c>}
	\end{split}
	\end{equation}
		\end{theorem}
		\begin{proof}
Так как связность инвариантна при инфинитезимальном преобразовании, мы имеем
	\begin{equation}
	\label{eq: Killing equation 2,1}
\mathcal{L}_\xi\overline{\Gamma^a_{bc}}=0
	\end{equation}
\eqref{eq: Killing equation 2} следует из
\eqref{eq: Killing equation 2,1} и \eqref{eq: Lie derivative of connection}.
		\end{proof}

Мы называем уравнение \eqref{eq: Killing equation 2}
\AddIndex{уравнением Килинга второго рода}{Killing equation second type}
и вектор $\xi^a$
\AddIndex{вектором Килинга второго рода}{Killing vector second type}.

		\begin{theorem}
Вектором Килинга второго рода удовлетворяет уравнению
	\begin{equation}
	\label{eq: Killing equation 2, colorary}
	\begin{split}
0&=\overline{R^a_{bcp}}\xi^p+\overline{R^a_{cpb}}\xi^p+\overline{R^a_{pbc}}\xi^p
\\ &+T^a_{bp;c}\xi^p+T^a_{pc;b}\xi^p
+T^p_{cb}\xi^a_{;<p>}
+T^a_{bp}\xi^p_{;<c>}
+T^a_{pc}\xi^p_{;<b>}
	\end{split}
	\end{equation}
		\end{theorem}
		\begin{proof}
Из \eqref{eq: Killing equation 2}
и \eqref{eq: commutator second derivative of vector}
следует, что
	\begin{equation}
	\label{eq: Killing equation 2,4}
	\begin{split}
\overline{R^a_{p bc}}\xi^p
-T^p_{bc}\xi^a_{;<p>}
&=\overline{R^a_{cbp}}\xi^p
+T^a_{cp;<b>}\xi^p
+T^a_{cp}\xi^p_{;<b>}\\
&-\overline{R^a_{bcp}}\xi^p
-T^a_{bp;<c>}\xi^p
-T^a_{bp}\xi^p_{;<c>}
	\end{split}
	\end{equation}
\eqref{eq: Killing equation 2, colorary} следует из \eqref{eq: Killing equation 2,4}.
		\end{proof}

		\begin{corollary}
Уравнением Килинга второго рода в римановом пространстве является тождеством.
Связность в римановом пространстве инвариагтна при
любом инфинитезимальном преобразовании \eqref{eq: infinitesimal displacement} 
		\end{corollary}
		\begin{proof}
Прежде всего, кручение равно 0. Остальное является следствием первого тождества Бианки.
		\end{proof}

			\section{Перенос Картана}
			\label{section: Cartan Transport}

Теоремы \ref{theorem: xtremeLine} и \ref{theorem: FrenetTransfer} утверждают, что
движение вдоль кривой порождает преобразование вектора, дополнительное
к параллельному переносу.
Это преобразование очень важно
и мы будем называть его \AddIndex{переносом Картана}{Cartan transport}.
Мы определим \AddIndex{символ Картана}{Cartan symbol}
\symb{\Gamma(C)^i_{kl}}0{Cartan symbol}
\[\ShowSymbol{Cartan symbol}=\frac 1 2 g^{im}(g_{kl;m}-g_{km;l}-g_{ml;k})\]
и \AddIndex{связность Картана}{Cartan connection}
\symb{\overbrace{\Gamma^i_{kl}}}0{overbrace Gamma i kl}
\[\ShowSymbol{overbrace Gamma i kl}
=\Gamma^i_{kl}-\Gamma(C)^i_{kl}
=\Gamma^i_{kl}-\frac 1 2 g^{im}(g_{kl;m}-g_{km;l}-g_{ml;k})\]
Пользуясь связностью Картана, мы можем записать перенос Картана в виде
\[da^i=-\overbrace{\Gamma^i_{kl}}a^k dx^l\]
Соответственно, мы определим
\AddIndex{производную Картана}{Cartan derivative}
\symb{\overbrace{\nabla_l} a^i}0{overbrace nabla_l}
\[\ShowSymbol{overbrace nabla_l}= a^i_{;\{l\}}=\partial_l a^i+\overbrace{\Gamma^i_{kl}}a^k\]
\symb{\overbrace{D} a^i}0{overbrace D}
\[\ShowSymbol{overbrace D}=da^i+\overbrace{\Gamma^i_{kl}}a^k dx^l\]

		\begin{theorem}
		\label{theorem: LengthTangentVector}
Перенос Картана вдоль экстремальной
кривой сохраняет длину касательного вектора.
		\end{theorem}
		\begin{proof}
Пусть $$v^i=\frac {dx^i}{ds}$$ - касательный вектор к экстремальной кривой.
Из теоремы \ref{theorem: xtremeLine} следует, что
$$\frac {Dv^l} {ds} =
\frac 1 2 g^{il} \left(g_{kj;i} - g_{ik;j}
- g_{ij;k}\right) v^k v^j
$$
и
$$\frac {Dg_{kl} v^k v^l}{ds}
= \frac {Dg_{kl}} {ds}v^k v^l
+ g_{kl}\frac {Dv^k} {ds} v^l
+ g_{kl}v^k \frac {Dv^l} {ds}=$$
$$= g_{kl;p}v^p v^k v^l+$$
$$+ g_{kl}g^{ik} \frac 1 2 \left(g_{rj;i} - g_{ir;j}
- g_{ij;r}\right) v^r v^j v^l+$$
$$+ g_{kl}v^k g^{il} \frac 1 2 \left(g_{rj;i} - g_{ir;j}
- g_{ij;r}\right) v^r v^j=$$
$$= g_{kl;p}v^p v^k v^l
+ \left(g_{rj;l} - g_{lr;j}
- g_{lj;r}\right) v^r v^j v^l = 0$$
Следовательно длина вектора $v^i$ не меняется вдоль экстремальной кривой.
		\end{proof}

Мы распространим перенос Картана на любой геометрический объект подобно тому, как мы это
делаем для параллельного переноса.

\begin{theorem}
\[
g_{ij;\{l\}}=0
\]
\end{theorem}

		\begin{proof}
\[
\overbrace{\nabla_l} g_{ij}=\partial_l g_{ij}
-\overbrace{\Gamma^k_{il}}g_{kj}
-\overbrace{\Gamma^k_{jl}}g_{ik}=
\]
\[
=g_{ij;l}
+\frac 1 2 g^{km}(g_{il;m}-g_{im;l}-g_{ml;i})g_{kj}
+\frac 1 2 g^{km}(g_{jl;m}-g_{jm;l}-g_{ml;j})g_{ik}=0
\]
		\end{proof}

Связность Картана $\overbrace{\Gamma^i_{kl}}$ отличается от связности $\Gamma^i_{kl}$
на дополнительное слагаемое, которое является симметричным тензором.
Для любой связности мы определяем стандартным образом производную и кривизну.
Утверждения геометрии и физики
имеют одну и ту же форму, независимо от того использую ли я связность $\Gamma^i_{kl}$ или связность Картана.
Чтобы это показать, мы можем обобщить понятие связности Картана
и изучать связность, определённую равенством
\symb{\overline{\Gamma^i_{kl}}}0{conection overline}
	\begin{equation}
\ShowSymbol{conection overline}=\Gamma^i_{kl}+A^i_{kl}
	\label{eq: conection overline}
	\end{equation}
где $A$ - это $0$, или символ Картана или любой другой
симметричный тензор.
Соответственно мы определяем производную
\symb{\overline{\nabla_l} a^i}0{overline nabla_l, definition 1}
\symb{a^i_{;<l>}}0{overline nabla_l, definition 2}
\[\ShowSymbol{overline nabla_l, definition 1}=
\ShowSymbol{overline nabla_l, definition 2}=
\partial_l a^i+\overline{\Gamma^i_{kl}}a^k\]
\symb{\overline{D} a^i}0{overline D}
\[\ShowSymbol{overline D}=da^i+\overline{\Gamma^i_{kl}}a^k dx^l\]
и кривизну
\symb{\overline{R^a_{bij}}}0{GLn curvature_overline}
	\begin{equation}
\ShowSymbol{GLn curvature_overline}
=\partial_i\overline{\Gamma^a_{bj}}-\partial_j\overline{\Gamma^a_{bi}}
+\overline{\Gamma^a_{ci}}\overline{\Gamma^c_{bj}}
-\overline{\Gamma^a_{cj}}\overline{\Gamma^c_{bi}}
	\label{eq: GLn curvature_overline}
	\end{equation}
Эта связность имеет тоже кручение
	\begin{equation}
T^a_{cb} =
\overline{\Gamma^a_{bc}}-\overline{\Gamma^a_{cb}}
\label{eq: Torsion coordinates_overline}
	\end{equation}

С этой точки зрения теорема \ref{theorem: LengthTangentVector} означает,
что экстремальная кривая является геодезической
для связности Картана.

		\begin{theorem}
		\label{theorem: curvature_overline}
Кривизна связности \eqref{eq: conection overline} имеет вид
	\begin{equation}
\overline{R^a_{bde}}=R^a_{bde}
+A^a_{be;d}-A^a_{bd;e}+A^a_{cd}A^c_{be}-A^a_{ce}A^c_{bd}+S^p_{de}A^a_{bp}
	\label{curvature_overline}
	\end{equation}
где $R^a_{bde}$ - кривизна связности $\Gamma^i_{kl}$
		\end{theorem}
		\begin{proof}
	\begin{align*}
\overline{R^a_{bde}}&=\overline{\Gamma^a_{be,d}}-\overline{\Gamma^a_{bd,e}}
+\overline{\Gamma^a_{cd}}\ \overline{\Gamma^c_{be}}-\overline{\Gamma^a_{ce}}\ \overline{\Gamma^c_{bd}}\\
&=\Gamma^a_{be,d}+A^a_{be,d}-\Gamma^a_{bd,e}-A^a_{bd,e}\\
&+(\Gamma^a_{cd}+A^a_{cd})(\Gamma^c_{be}+A^c_{be})-(\Gamma^a_{ce}+A^a_{ce})(\Gamma^c_{bd}+A^c_{bd})\\
&=\Gamma^a_{be,d}+A^a_{be,d}-\Gamma^a_{bd,e}-A^a_{bd,e}\\
&+\Gamma^a_{cd}\Gamma^c_{be}+\Gamma^a_{cd}A^c_{be}+A^a_{cd}\Gamma^c_{be}+A^a_{cd}A^c_{be}\\
&-\Gamma^a_{ce}\Gamma^c_{bd}-A^a_{ce}\Gamma^c_{bd}-\Gamma^a_{ce}A^c_{bd}-A^a_{ce}A^c_{bd}\\
&=R^a_{bde}+A^a_{be,d}-A^a_{bd,e}\\
&+\Gamma^a_{cd}A^c_{be}+A^a_{cd}\Gamma^c_{be}+A^a_{cd}A^c_{be}\\
&-A^a_{ce}\Gamma^c_{bd}-\Gamma^a_{ce}A^c_{bd}-A^a_{ce}A^c_{bd}\\
&=R^a_{bde}\\
&+A^a_{be;d}-\underline{\Gamma^a_{pd}A^p_{be}}_2+\underline{\Gamma^p_{bd}A^a_{pe}}_4+\underline{\Gamma^p_{ed}A^a_{bp}}_{1:S}\\
&-A^a_{bd;e}+\underline{\Gamma^a_{pe}A^p_{bd}}_3-\underline{\Gamma^p_{be}A^a_{pd}}_5-\underline{\Gamma^p_{de}A^a_{bp}}_1\\
&+\underline{\Gamma^a_{cd}A^c_{be}}_2+\underline{\Gamma^c_{be}A^a_{cd}}_5+A^a_{cd}A^c_{be}\\
&-\underline{\Gamma^c_{bd}A^a_{ce}}_4-\underline{\Gamma^a_{ce}A^c_{bd}}_3-A^a_{ce}A^c_{bd}
	\end{align*}
		\end{proof}

		\begin{corollary}
\AddIndex{Кривизна Картана}{Cartan curvature} имеет вид
\symb{\overbrace{R^a_{bde}}}0{Cartan curvature}
	\begin{equation}
	\begin{split}
\ShowSymbol{Cartan curvature}&=R^a_{bde}
-\Gamma(C)^a_{be;d}+\Gamma(C)^a_{bd;e}\\
&+\Gamma(C)^a_{cd}\Gamma(C)^c_{be}-\Gamma(C)^a_{ce}\Gamma(C)^c_{bd}-T^p_{de}\Gamma(C)^a_{bp}
	\end{split}
	\label{eq: Cartan curvature}
	\end{equation}
		\end{corollary}


==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{texSpaceTime}{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84 (1966)
}%

\BiblioItem{texGenRelativity}{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{texGenRelativity}{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{texAffine,texGeomObject}{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{texAffine}{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{texAffine}{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{texAffine}{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\BiblioItem{texAffine}{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%

\BiblioItem{texTidal,texAffine,texGeomObject}{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{texTidal,texNewton}{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{texNewton}{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{texNewton}{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{texLagrange}{Weinberg}
{
Steven Weinberg. The Quantum Theory of Fields. Cambridge university press.
}%

\BiblioItem{texLagrange}{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{texLagrange}{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{texTidal}{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{texPrefaceTidal,texPrefaceRefernceFrame}{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{texTidal}{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{texReferenceFrame,texFiberedAlgebra}{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{texFiberedAlgebra,texTstarMorphism}{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{texGeomObject}{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{texAffine,texRepresentation,texBasis,texDrcBasis,texVectorSpace,texLinearMap,texPolyvector}
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem{texPolyvector}{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{texDrcBasis,texBasis}{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{texBundle}{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{texPrefaceRefernceFrame}{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{texPrefaceRefernceFrame}{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{texPrefaceRefernceFrame}{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{texPrefaceRefernceFrame}{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{texPrefaceRefernceFrame}{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{texPrefaceRefernceFrame}{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texPrefaceRefernceFrame}{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texPrefaceRefernceFrame,texPrefaceTidal}{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{texBiring,texVectorSpace}{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{texBiring,texVectorSpace}
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{texVectorSpace}{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{texVectorSpace}{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{texVectorSpace}{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{texVectorSpace}{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{texDrcReferenceFrame,texRefernceFrame,texLie,texLieRepresentation}{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2004)
}%

\BiblioItem{texAffine}{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2004)
}%

\BiblioItem{texTidal}{0405.028}
{
Aleks Kleyn, Metric\hyph Affine Manifold,
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2004)
}%

\BiblioItem{texFiberedAlgebra,texBundleRelation,texTstarMorphism}{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2007)
}%

\BiblioItem{texBundleRelation,texPrefaceRelation}{0702.561}
{
Александр Клейн,
Расслоенная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

%\BiblioItem{texBasis,texLinearMap}{math.RA-0501237}
%{
%Александр Клейн,
%Векторное пространство над телом,\\
%eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2005)
%}%

\BiblioItem{texPolymodule}{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Skew-Field, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\ifx\texBiring\Defined
\else
\BiblioItem{texVectorSpace,texFiberedAlgebra}{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2006)
}%
\fi

\ifx\texBundleRelation\Defined
\else
\BiblioItem{texFiberedMorphism}{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%
\fi

\ifx\PrintBook\Defined
\BiblioItem{texPrefaceRelation}{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%
\fi

\BiblioItem{texHomotopy}{q-alg-9705009}
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{texSpaceTime}{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81 (1967)
}%

\BiblioItem{texPrefaceRelation}{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem{texBundleRelation,texPrefaceRelation,texTstarMorphism,texBundle}
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem{texBundle}
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{texFiberedAlgebra}{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{texBundleRelation}{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{texBundle,texCartesian,texFiberedAlgebra,texBundleRelation,texFiberedMorphism}
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{texCalculus}{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{texCalculus}{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{texCalculus}{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem{texFiberedMorphism}{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{texFiberedAlgebra,texFiberedMorphism}{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{texFiberedMorphism}{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{texFiberedMorphism}{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{texPolyvector}{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\CloseBiblio



==> Geom.Object.Russian.tex <==
%auto-ignore
\def\texGeomObject{}
\ifx\PrintBook\Defined
				\chapter{Геометрический объект}
\fi

			\section{Метрико-аффинное многообразие}
			\label{section: Metric-affine Manifold}

В случае связности \xEqRef{0405.027}{eq: GLn connection form}
мы определим \AddIndex{форму кручение}{torsion form}
	\begin{equation}
T^a = d^2 x^a + \omega^a_b \wedge dx^b
	\label{eq: Torsion}
	\end{equation}
Из \xEqRef{0405.027}{eq: GLn connection form} следует
	\begin{equation}
\omega^a_b \wedge dx^b=(\Gamma^a_{bc}-\Gamma^a_{cb})dx^c\wedge dx^b
	\label{eq: wedge connection}
	\end{equation}
Подставляя \eqref{eq: wedge connection} и \xEqRef{0405.027}{eq: anholonomity} в \eqref{eq: Torsion}
мы получим
	\begin{equation}
T^a=T^a_{cb}dx^c\wedge dx^b =
-c^a_{cb}dx^c\wedge dx^b + (\Gamma^a_{bc}-\Gamma^a_{cb})dx^c\wedge dx^b
\label{eq: Torsion 1}
	\end{equation}
где мы определили \AddIndex{тензор кручение}{torsion tensor}
	\begin{equation}
T^a_{cb} =
\Gamma^a_{bc}-\Gamma^a_{cb}-c^a_{cb}
\label{eq: Torsion coordinates}
	\end{equation}

Коммутатор вторых производных имеет вид
	\begin{equation}
u^\alpha_{;kl}-u^\alpha_{;lk}
=R^\alpha_{\beta lk}u^\beta
-T^p_{lk}u^\alpha_{;p}
	\label{eq: commutator second derivative}
	\end{equation}
Из \eqref{eq: commutator second derivative} следует, что
	\begin{equation}
	\label{eq: commutator second derivative of vector}
\xi^a_{;cb}-\xi^a_{;bc}
=R^a_{d bc}\xi^d
-T^p_{bc}\xi^a_{;p}
	\end{equation}

В римановом пространстве мы have metric tensor $g_{ij}$ и связность $\Gamma^k_{ij}$.
Одно из свойств риманова пространства - это симметрия связности и равенство нулю ковариантной производной
метрики. Это порождает тесную связь между метрикой и связностью.
However  связность is not necessarily symmetric
и ковариантная производная метрического тензора может быть отлична от 0.
В последнем случае мы вводим \AddIndex{неметричность}{nonmetricity}
	\begin{equation}
Q^{ij}_k=g^{ij}_{;k}=g^{ij}_{,k}+\Gamma^i_{pk}g^{pj}+\Gamma^j_{pk}g^{ip}
	\label{eq: Nonmetricity}
	\end{equation}

Так как производная метрического тензора не равна 0, мы не можем поднимать или опускать индекс
тензора внутри производной как мы это делаем в обычном римановом пространстве.
Теперь эта операция принимает следующий вид
\[a^i_{;k} = g^{ij} a_{j;k} + g^{ij}_{;k} a_j\]
Это равенство для метрического тензора принимает следующий вид
\[g^{ab}_{;k} = - g^{ai} g^{bj} g_{ij;k}\]

		\begin{definition}
Мы будем называть многообразие с кручением
и неметричностью
\AddIndex{метрико\Hyph аффинным многообразием}{metric-affine manifold} \citeBib{Mielke}.
		\qed  
		\end{definition}

Если мы изучаем подмногообразие $V_n$ многообразия $V_{n+m}$, мы видим, что имерсия порождает
связность $\Gamma^\alpha_{\beta\gamma}$, которая связана со связностью в многообразии соотношением
\[
\Gamma^\alpha_{\beta\gamma} e^l_\alpha =
\Gamma^l_{mk} e^m_\beta e^k_\gamma + \frac {\partial e^l_\beta} {\partial u^\gamma}
\]
Следовательно, не существует непрерывного вложения
пространства с кручением в риманово пространство.

			\section{Геометрический смысл кручения}

Предположим, что $a$ и $b$ - неколинеарные векторы в точке $A$ (см. фиг. \ref{fig:Torsion}).

%\begin{table}[h]
\begin{tabular}{l|r}
\begin{minipage}{160pt}
Мы проведём геодезическую $L_a$ через точку $A$, используя вектор $a$
как касательный вектор к $L_a$ в точке $A$.
Пусть $\tau$ - канонический параметр на $L_a$ и
\[\frac {dx^k}{d\tau}=a^k\]
Мы перенесём вектор $b$ вдоль геодезической $L_a$ из точки $A$
в точку $B$, определённую значением параметра $\tau=\rho>0$. Мы обозначим результат $b'$.
\end{minipage}
&
\begin{minipage}{160pt}
Мы проведём геодезическую $L_b$ через точку $A$, используя вектор $b$
как касательный вектор к $L_b$ в точке $A$.
Пусть $\varphi$ - канонический параметр на $L_b$ и
\[\frac {dx^k}{d\varphi}=b^k\]
Мы перенесём вектор $a$ вдоль геодезической $L_b$ из точки $A$
в точку $D$, определённую значением параметра $\varphi=\rho>0$. Мы обозначим результат $a'$.
\end{minipage}
\end{tabular}
%\end{table}

%\begin{table}[h]
\begin{tabular}{l|r}
\begin{minipage}{160pt}
Мы проведём геодезическую $L_{b'}$ через точку $B$, используя вектор $b'$
как касательный вектор к $L_{b'}$ в точке $B$.
Пусть $\varphi'$ - канонический параметр на $L_{b'}$ и 
\[\frac {dx^k}{d\varphi'}=b'^k\]
Мы определим точку $C$ на геодезической $L_{b'}$ значением параметра $\varphi'=\rho$
\end{minipage}
&
\begin{minipage}{160pt}
Мы проведём геодезическую $L_{a'}$ через точку $D$, используя вектор $a'$
как касательный вектор к $L_{a'}$ в точке $D$.
Пусть $\tau'$ - канонический параметр на $L_{a'}$ и 
\[\frac {dx^k}{d\tau'}=a'^k\]
Мы определим точку $E$ на геодезической $L_{a'}$ значением параметра $\tau'=\rho$
\end{minipage}
\end{tabular}
%\end{table}

Формально линии $AB$ и $DE$ так же, как линии $AD$ и $BC$, параллельны.
Длины отрезков $AB$ и $DE$ равны так же, как длины
отрезков $AD$ и $BC$ равны. Мы называем такую фигуру
\AddIndex{параллелограммом}{parallelogram}, построенным на векторах
$a$ и $b$ с вершиной в точке $A$.

		\begin{theorem}
Предположим $CBADE$ - параллелограм с вершиной в точке
$A$; тогда построенная фигура не будет замкнута \citeBib{torsion}.
Величина различия координат
точек $C$ и $E$ равна поверхностному интегралу кручения
над этим параллелограммом\footnote{Доказательство этого утверждения я нашёл в \citeBib{Shilov}}
\[\Delta_{CE}x^k=\iint T^k_{mn}dx^m \wedge dx^n \]
		\end{theorem}

	\begin{figure}
	\begin{center}
	\begin{picture}(150,150)
\put( 20, 25){ $A$ }
\put( 30, 65){ $a$ }
\put( 45, 50){ $b$ }
\put( 55, 130){ $B$ }
\put( 80, 135){ $b'$ }
\put( 155, 80){ $a'$ }
\put( 165, 150){ $C$ }
\put( 170, 40){ $D$ }
\put( 195, 135){ $E$ }
\put(-115, -65){\qbezier(150,100)(162,150)(185,190)}%AB
\put(35, 35){\vector(1,4){11}}%a
%\put(35, 35){\line(2, 5){36}}%AB
\put(-115, -65){\qbezier(185,190)(218,207)(283,210)}%BC
\put(70, 125){\vector(2,1){30}}%b'
%\put(70, 125){\line(5, 1){98}}%BC
\put(169, 145){\line(3, -2){18}}%CE
\put(-149, -154){\qbezier(320,212)(323,260)(336,287)}%DE
\put(171, 59){\vector(0,1){35}}%a'
%\put(174, 59){\line(1, 6){12.4}}%DE
\put(-149, -154){\qbezier(185,190)(208,206)(320,212)}%AD
\put(35, 35){\vector(3,2){30}}%b
%\put(35, 35){\line(6, 1){139}}%AD
	\end{picture}
	\caption{Meaning of Torsion}
	\label{fig:Torsion}
	\end{center}
	\end{figure}
		\begin{proof}
Мы можем найти приращение координаты $x^k$ вдоль геодезической в виде
	\begin{align*}
\Delta x^k&=\frac{dx^k}{d\tau}\tau+\frac 1 2 \frac{d^2 x^k}{d\tau^2}\tau^2+O(\tau^2)=\\
&=\frac{dx^k}{d\tau}\tau-\frac 1 2 \Gamma^k_{mn}\frac{dx^m}{d\tau} \frac{dx^n}{d\tau}\tau^2+O(\tau^2)
	\end{align*}
где $\tau$ - канонический параметр и мы вычисляем производные и компоненты
$\Gamma^k_{mn}$ в начальной точке. В частности 
	\[
\Delta_{AB} x^k=a^k\rho-\frac 1 2 \Gamma^k_{mn}(A)a^m a^n\rho^2+O(\rho^2)
	\]
вдоль геодезической $L_a$ и
	\begin{equation}
\Delta_{BC} x^k=b'^k\rho-\frac 1 2 \Gamma^k_{mn}(B)b'^m b'^n\rho^2+O(\rho^2)
	\label{eq:Torsion_1}
	\end{equation}
вдоль геодезической $L_{b'}$. Здесь
	\begin{equation}
b'^k=b^k- \Gamma^k_{mn}(A)b^m dx^n+O(dx)
	\label{eq:Torsion_2}
	\end{equation}
результат параллельного переноса $b^k$ из $A$ в $B$ и
	\begin{equation}
dx^k=\Delta_{AB} x^k=a^k\rho
	\label{eq:Torsion_3}
	\end{equation}
с точностью до малой первого порядка. Подставляя
\eqref{eq:Torsion_3} в \eqref{eq:Torsion_2} и \eqref{eq:Torsion_2} в
\eqref{eq:Torsion_1}, мы получим
\[
\Delta_{BC} x^k=b^k \rho- \Gamma^k_{mn}(A)b^m a^n \rho^2
-\frac 1 2 \Gamma^k_{mn}(B)b^m b^n\rho^2+O(\rho^2)
\]
Общее приращение координаты $x^K$ вдоль пути $ABC$ имеет вид
\[
\Delta_{ABC}x^k=\Delta_{AB} x^k+\Delta_{BC} x^k=
\]
	\begin{equation}
	\label{eq:Torsion_4}
=(a^k+b^k)\rho- \Gamma^k_{mn}(A)b^m a^n \rho^2-
	\end{equation}
\[
-\frac 1 2 \Gamma^k_{mn}(B)b^m b^n\rho^2
-\frac 1 2 \Gamma^k_{mn}(A)a^m a^n\rho^2+O(\rho^2)
\]

Аналогично общее приращение координаты $x^K$ вдоль пути $ADE$ имеет вид
\[
\Delta_{ADE}x^k=\Delta_{AD} x^k+\Delta_{DE} x^k=
\]
	\begin{equation}
	\label{eq:Torsion_5}
=(a^k+b^k)\rho- \Gamma^k_{mn}(A)a^m b^n \rho^2-
	\end{equation}
\[
-\frac 1 2 \Gamma^k_{mn}(D)a^m a^n\rho^2
-\frac 1 2 \Gamma^k_{mn}(A)b^m b^n\rho^2+O(\rho^2)
\]

Из \eqref{eq:Torsion_4} и \eqref{eq:Torsion_5} следует, что
\[
\Delta_{ADE}x^k-\Delta_{ABC}x^k=\]
\[= \Gamma^k_{mn}(A)b^m a^n\rho^2
+\underline{\frac 1 2 \Gamma^k_{mn}(B)b^m b^n\rho^2}_1
+\underline{\frac 1 2 \Gamma^k_{mn}(A)a^m a^n\rho^2}_2-\]
\[- \Gamma^k_{mn}(A)a^m b^n \rho^2
-\underline{\frac 1 2 \Gamma^k_{mn}(D)a^m a^n\rho^2}_2
-\underline{\frac 1 2 \Gamma^k_{mn}(A)b^m b^n\rho^2}_1+O(\rho^2)
\]
Для достаточно малого значения $\rho$ подчёркнутые слагаемые взаимно уничтожаются
и мы получаем интегральную сумму для выражения
\[
\Delta_{ADE}x^k-\Delta_{ABC}x^k=\iint_\Sigma (\Gamma^k_{nm}- \Gamma^k_{mn})dx^m \wedge dx^n
\]

Однако недостаточно найти разность
\[\Delta_{ADE}x^k-\Delta_{ABC}x^k\]
чтобы найти разность координат точек $C$ и $E$.
Координаты могут быть неголономными и мы должны учесть, что
координаты вдоль замкнутого пути изменяются \xEqRef{0405.027}{eq: change of coordinate along a loop}
\[\Delta x^k=\oint_{ECBADE}dx^k=-\iint_\Sigma c^k_{mn}dx^m \wedge dx^n \]
где $c$ - объект неголономности.

Окончательно разность координат точек $C$ и $E$ имеет вид
\[\Delta_{CE}x^k=\Delta_{ADE}x^k-\Delta_{ABC}x^k+\Delta x^k=
\iint_\Sigma (\Gamma^k_{nm}- \Gamma^k_{mn}-c^k_{mn})dx^m \wedge dx^n\]
Используя \eqref{eq: Torsion coordinates}, мы доказали утверждение. 
		\end{proof}

			\section{Соотношение между связностью и метрикой}

Сейчас мы хотим найти, как мы можем выразить связность, если известны
метрика и кручение. Согласно определению
\[-Q_{kij}=g_{ij;k}=g_{ij,k}-\Gamma^p_{ik}g_{pj}-\Gamma^p_{jk}g_{pi}\]
\[-Q_{kij}=g_{ij,k}-\Gamma^p_{ik}g_{pj}-\Gamma^p_{kj}g_{pi}-S^p_{jk}g_{pi}\]
Перенесём производную $g$ и кручение в левую часть.
	\begin{equation}
g_{ij,k}+Q_{kij}-S^p_{jk}g_{pi}=\Gamma^p_{ik}g_{pj}+\Gamma^p_{kj}g_{pi}
	\label{eq: Connection1}
	\end{equation}
Меняя порядок индексов, мы запишем ещё два уравнения
	\begin{equation}
g_{jk,i}+Q_{ijk}-S^p_{ki}g_{pj}=\Gamma^p_{ji}g_{pk}+\Gamma^p_{ik}g_{pj}
	\label{eq: Connection2}
	\end{equation}
	\begin{equation}
g_{ki,j}+Q_{jki}-S^p_{ij}g_{pk}=\Gamma^p_{kj}g_{pi}+\Gamma^p_{ji}g_{pk}
	\label{eq: Connection3}
	\end{equation}
Если мы вычтем равенство \eqref{eq: Connection1} из суммы равенств
\eqref{eq: Connection2} и \eqref{eq: Connection1}, то мы получим
\[
g_{ki,j}+g_{jk,i}-g_{ij,k}+Q_{ijk}+Q_{jki}-Q_{kij}
-S^p_{ij}g_{pk}-S^p_{ki}g_{pj}+S^p_{jk}g_{pi}=2\Gamma^p_{ji}g_{pk}
\]
Окончательно мы получаем
\[
\Gamma^p_{ji}=\frac 1 2 g^{pk}
(g_{ki,j}+g_{jk,i}-g_{ij,k}+Q_{ijk}+Q_{jki}-Q_{kij}
-S^r_{ij}g_{rk}-S^r_{ki}g_{rj}+S^r_{jk}g_{ri})
\]


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index{texLinearMap}%1%1
   {$1$-\drc форма}%
   {1-drc form, vector spaces}%
\SetIndexSpace%
\Index{texPolymodule}%2%66
   {$(2)$\hyph векторное пространство}%
   {(2)-vector space}%
\Index{texBundleRelation}%2%122
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index{texBiring}%A%2
   {$(^{\gi a}_{\gi b})$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index{texBiring}%A%34
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant}%
\Index{texCalculus}%A%67
   {$A$\Hyph значная функция}%
   {A valued function}%
\SetIndexSpace%
\Index{texBiring}%C%3
   {\subs строка матрицы}%
   {c row}%
\Index{texVectorSpace}%C%5
   {\CR матричная группа}%
   {cr-matrix group}%
\Index{texBiring}%C%6
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index{texBiring}%C%7
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index{texBiring}%C%8
   {\CR степень}%
   {cr power}%
\Index{texVectorSpace}%C%9
   {\crd векторное пространство}%
   {crd vector space}%
\Index{texBiring}%C%10
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index{texVectorSpace}%D%11
   {\dcr базис векторного пространства \subs строк}%
   {dcr basis, c rows vector space}%
\Index{texVectorSpace}%D%12
   {\dcr вектор}%
   {dcr vector}%
\Index{texVectorSpace}%D%13
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index{texVectorSpace}%D%14
   {\dcr векторное пространство \subs строк}%
   {subs rows dcr vector space}%
\Index{texVectorSpace}%D%15
   {\drc  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index{texVectorSpace}%D%55
   {\drc автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index{texVectorSpace}%D%17
   {\drc базис}%
   {}%
\SubIndex{texVectorSpace}%4%
   {в векторном пространстве}%
   {drc basis, vector space}%
\SubIndex{texVectorSpace}%5%
   {в векторном пространстве \sups строк}%
   {drc basis, r rows vector space}%
\Index{texVectorSpace}%D%18
   {\drc вектор}%
   {drc vector}%
\Index{texVectorSpace}%D%19
   {\drc векторное пространство}%
   {drc vector space}%
\Index{texVectorSpace}%D%20
   {\drc векторное пространство \sups строк}%
   {sups rows drc vector space}%
\Index{texCalculus}%D%46
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index{texVectorSpace}%D%83
   {\drc изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index{texVectorSpace}%D%87
   {\drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Index{texVectorSpace}%D%23
   {\drc линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index{texVectorSpace}%D%114
   {\drc линейно независимые векторы}%
   {linearly independent, vector space}%
\Index{texDrcMorphism}%D%25
   {\drc линейное отображение векторных пространств}%
   {drc linear map of vector spaces}%
\Index{texVectorSpace}%D%27
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index{texVectorSpace}%D%26
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index{texCalculus}%D%96
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\SetIndexSpace%
\Index{texELie}%E%28
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index{texDiffEq}%E%29
   {essential parameters}%
   {essential parameters}%
\SetIndexSpace%
\Index{texRefernceFrame}%G%205
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index{texTypeBasis}%G%30
   {\Gbasis}%
   {G-basis}%
\Index{texTypeBasis}%G%31
   {\Gcoords ы}%
   {G-coordinates}%
\Index{texTypeBasis}%G%32
   {\Gspace о}%
   {GSpace}%
\Index{texBasis}%G%267
   {\Gbasis\ векторного пространства}%
   {G-basis}%
\Index{texBasis}%G%270
   {\Gcoords ы базиса}%
   {G-coordinates}%
\Index{texBasis}%G%271
   {\Gspace о}%
   {GSpace}%
\SetIndexSpace%
\Index{texPolyvector}%M%361
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\Index{texPolyvector}%M%24
   {$m$\Hyph вектор}%
   {m-vector}%
\SetIndexSpace%
\Index{texPolymodule}%N%231
   {$(n)$\hyph векторное пространство}%
   {(n)-vector space}%
\Index{texBundleRelation}%N%218
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index{texBiring}%R%35
   {\sups строка матрицы}%
   {r row}%
\Index{texVectorSpace}%R%36
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index{texVectorSpace}%R%37
   {\RC главный минор}%
   {RC-major minor}%
\Index{texBiring}%R%38
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index{texVectorSpace}%R%39
   {\RC матричная группа}%
   {rc-matrix group}%
\Index{texVectorSpace}%R%40
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index{texBiring}%R%41
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index{texBiring}%R%42
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index{texVectorSpace}%R%43
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index{texBiring}%R%44
   {\RC степень}%
   {rc power}%
\Index{texVectorSpace}%R%45
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index{texVectorSpace}%R%213
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index{texBiring}%R%47
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index{texDrcMorphism}%S%314
   {$(S\RCstar,T\RCstar)$\Hyph линейное отображение векторных пространств}%
   {src trc linear map of vector spaces}%
\Index{texLinearMap}%S%48
   {$\star D$\Hyph произведением \drc линейного отображения $A$ на скаляр}%
   {starD product of drc linear map over scalar}%
\Index{texVectorSpace}%S%217
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index{texVectorSpace}%S%216
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index{texTstarRepresentation}%S%49
   {\sT сдвиг}%
   {starT shift}%
\Index{texFiberedGroup}%S%50
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\Index{texTstarMorphism}%S%160
   {\sT представление $\mathfrakl{F}$\Hyph алгебры $A$ в множестве $M$}%
   {starT representation of algebra}%
\Index{texFiberedAlgebra}%S%162
   {\sT представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {starT representation of fibered F-algebra}%
\Index{texFiberedGroup}%S%163
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index{texTstarMorphism}%S%308
   {\sT преобразование}%
   {starT transformation}%
\Index{texFiberedAlgebra}%S%167
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\SubIndex{}%71%
   {невырожденное}%
   {nonsingular transformation of bundle}%
\SetIndexSpace%
\Index{texVectorSpace}%T%51
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index{texVectorSpace}%T%52
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index{texFiberedGroup}%T%316
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\Index{texTstarRepresentation}%T%53
   {\Ts сдвиг}%
   {Tstar shift}%
\Index{texTstarMorphism}%T%301
   {\Ts представление $\mathfrakl{F}$\Hyph алгебры $A$ в множестве $M$}%
   {Tstar representation of algebra}%
\Index{texFiberedAlgebra}%T%321
   {\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {Tstar representation of fibered F-algebra}%
\Index{texTstarMorphism}%T%309
   {\Ts преобразование}%
   {Tstar transformation}%
\Index{texFiberedAlgebra}%T%327
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\SetIndexSpace%
\Index{texAffine}%А%56
   {автопараллельная кривая}%
   {auto parallel line}%
\Index{texDrcBasis}%А%57
   {активное \sT представление}%
   {active representation, vector space}%
\Index{texBasis}%А%262
   {активное представление}%
   {active representation}%
\Index{texBasis}%А%263
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index{texLie}%А%58
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\SubIndex{texLie}%9%
   {определённая слева}%
   {left defined algebra Lie}%
\SubIndex{texLie}%10%
   {определённая справа}%
   {right defined algebra Lie}%
\Index{texBiring}%А%59
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index{texFiberedGroup}%А%60
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index{texBundleRelation}%А%156
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index{texFiberedAlgebra}%А%61
   {арность операции}%
   {arity of operation}%
\Index{texBasis}%А%277
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index{texBasis}%А%275
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index{texBundle}%Б%172
   {база отображения}%
   {base of map}%
\Index{texBundleRelation}%Б%233
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index{texTypeBasis}%Б%16
   {базис}%
   {}%
\SubIndex{texTypeBasis}%1%
   {аффинный}%
   {Affine Basis}%
\SubIndex{texTypeBasis}%2%
   {ортонормальный}%
   {Orthonornal Basis}%
\SubIndex{texTypeBasis}%3%
   {центро-аффинный}%
   {Central Affine Basis}%
\Index{texBasis}%Б%266
   {базис векторного пространства}%
   {Basis}%
\Index{texLieRepresentation}%Б%62
   {базовый вектор}%
   {}%
\SubIndex{texLieRepresentation}%11%
   {\sT представления}%
   {basis vector of starT representation}%
\SubIndex{texLieRepresentation}%12%
   {\Ts представления}%
   {basis vector of Tstar representation}%
\Index{texLie}%Б%63
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index{texFiberedMorphism}%Б%351
   {башня расслоений}%
   {tower of bundles}%
\Index{texLieRepresentation}%Б%64
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index{texBiring}%Б%65
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index{texPolymodule}%В%230
   {($D_1\RCstar$, ..., $D_n\RCstar$)\hyph векторное пространство}%
   {(d1rc,dnrc)-vector space}%
\Index{texPolymodule}%В%229
   {($S\star$, $\star T$)\hyph векторное пространство}%
   {(Sstar,starT)-vector space}%
\Index{texDiffProperty}%В%69
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index{texRepresentation}%В%261
   {вектор\hyph столбец}%
   {column vector}%
\Index{texFiberedAlgebra}%В%70
   {векторное расслоение}%
   {vector bundle}%
\Index{texNewton}%В%54
   {векторный потенциал}%
   {vector potential}%
\Index{texRepresentation}%В%260
   {вектор\hyph строка}%
   {row vector}%
\Index{texDiffEq}%В%71
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index{texNewton}%В%72
   {второй закон Ньютона}%
   {Second Newton law}%
\SetIndexSpace%
\Index{texDrcBasis}%Г%73
   {геометрический объект}%
   {}%
\SubIndex{texDrcBasis}%13%
   {в координатном представлении,	определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\SubIndex{texDrcBasis}%14%
   {определённый в векторном пространстве}%
   {geometrical object, vector space}%
\SubIndex{texDrcBasis}%15%
   {типа $A$}%
   {geometrical object of type A, vector space}%
\Index{texBasis}%Г%290
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%
\Index{texBasis}%Г%288
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Index{texBasis}%Г%293
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometrical object of type A, vector space}%
\Index{texRefernceFrame}%Г%74
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index{texRefernceFrame}%Г%195
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index{texFiberedAlgebra}%Г%75
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Index{texFiberedGroup}%Г%76
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index{texTypeBasis}%Г%77
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%274
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%264
   {группа симметрии}%
   {symmetry group}%
\Index{texDrcBasis}%Г%78
   {группа симметрии}%
   {SymmetryGroup}%
\Index{texTstarRepresentation}%Г%344
   {группа стабилизации}%
   {stability group}%
\Index{texGroupRing}%Г%79
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index{}%Д%283
   {движение на многообразии базисов}%
   {movement transformation}%
\Index{texBundle}%Д%331
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index{texBundle}%Д%357
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power of bundle}%
\Index{texCartesian}%Д%176
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Index{texCartesian}%Д%180
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index{texCartesian}%Д%181
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index{texBundleRelation}%Д%113
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index{texBundleRelation}%Д%227
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index{texCalculus}%Д%105
   {дифференциал отображения нормированного \drc векторного пространства в нормированное тело}%
   {differential, drc vector space to skew field}%
\Index{texCalculus}%Д%99
   {дифференцируемая функция \drc векторного пространства в тело $D$ }%
   {differentiable functions, drc vector space to skew field}%
\SetIndexSpace%
\Index{texDrcMorphism}%З%312
   {закон ассоциативности для \drc линейных отображений векторных пространств}%
   {associative law for drc linear maps of vector spaces}%
\Index{texVectorSpace}%З%310
   {закон ассоциативности для \Ts векторного пространства}%
   {associative law, Tstar vector space}%
\Index{texTstarRepresentation}%З%80
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for Tstar covariant representation}%
\Index{texLinearMap}%З%311
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index{texBundleRelation}%З%155
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index{texVectorSpace}%З%81
   {закон дистрибутивности}%
   {}%
\SubIndex{texVectorSpace}%20%
   {\Ts векторное пространство}%
   {distributive law, Tstar vector space}%
\Index{texVectorSpace}%З%82
   {закон унитарности}%
   {}%
\SubIndex{texVectorSpace}%21%
   {для \Ts векторного пространства}%
   {unitarity law, Tstar vector space}%
\SetIndexSpace%
\Index{texFiberedAlgebra}%И%84
   {изоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {isomorphism of fibered F-algebras}%
\Index{texLinearLie}%И%85
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index{texHomotopy}%К%4
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index{texBundleRelation}%К%111
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index{texBundleRelation}%К%112
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index{texBasis}%К%278
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index{texBasis}%К%284
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index{texFiberedGroup}%К%318
   {ковариантное \Ts представление расслоенной группы}%
   {Tstar covariant representation of fibered group}%
\Index{texBundleRelation}%К%228
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index{texBundle}%К%332
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index{texFiberedGroup}%К%317
   {контравариантное \Ts представление расслоенной группы}%
   {Tstar contravariant representation of fibered group}%
\Index{texVectorSpace}%К%21
   {координатная матрица}%
   {}%
\SubIndex{texVectorSpace}%6%
   {вектора в \drc базисе}%
   {coordinate matrix of vector in drc basis}%
\SubIndex{texVectorSpace}%7%
   {множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\SubIndex{texVectorSpace}%8%
   {множества векторов в векторном пространстве \drc строк}%
   {coordinate matrix of set of vectors, drc vector space}%
\Index{texRefernceFrame}%К%86
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index{texBasis}%К%285
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index{texDrcBasis}%К%88
   {координатное представление в \drc векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%287
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%286
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%89
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%22
   {координаты вектора в \drc базисе}%
   {coordinates of vector in drc basis}%
\Index{texDrcBasis}%К%90
   {координаты геометрического объекта}%
   {}%
\SubIndex{texDrcBasis}%22%
   {в векторном пространстве}%
   {coordinates of geometrical object, vector space}%
\SubIndex{texDrcBasis}%23%
   {в координатном векторном пространстве}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texBasis}%К%291
   {координаты геометрического объекта}%
   {coordinates of geometrical object, vector space}%
\Index{texBasis}%К%289
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texVectorSpace}%К%91
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index{texVectorSpace}%К%92
   {координаты множества векторов в \drc векторном пространстве}%
   {coordinates of set of vectors, drc vector space}%
\Index{texDrcBasis}%К%93
   {координаты представления}%
   {coordinates of representation}%
\Index{texBasis}%К%265
   {координаты представления}%
   {coordinates of representation}%
\Index{texPolyvector}%К%360
   {косое произведение векторов}%
   {skew product of vectors}%
\Index{texAffine}%К%94
   {кривизна Картана}%
   {Cartan curvature}%
\SetIndexSpace%
\Index{texVectorSpace}%Л%98
   {левое векторное пространство}%
   {left vector space}%
\Index{texLie}%Л%101
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index{texRepresentation}%Л%247
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation}%
\Index{texRepresentation}%Л%249
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation}%
\Index{texTstarMorphism}%Л%302
   {левостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {left-side representation of algebra}%
\Index{texRepresentation}%Л%244
   {левостороннее представление группы}%
   {left-side representation of group}%
\Index{texFiberedAlgebra}%Л%322
   {левостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {left-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%Л%164
   {левостороннее преобразование}%
   {left-side transformation}%
\Index{texFiberedAlgebra}%Л%328
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index{texLie}%Л%103
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index{texVectorSpace}%Л%214
   {левый модуль}%
   {left module}%
\Index{texTstarRepresentation}%Л%108
   {левый сдвиг}%
   {left shift}%
\Index{texRepresentation}%Л%251
   {левый сдвиг на группе}%
   {left shift, group}%
\Index{texFiberedGroup}%Л%109
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index{texRepresentation}%Л%240
   {линейное представление группы}%
   {linear representation of group}%
\Index{texBundle}%Л%116
   {лифт отображения}%
   {lift of map}%
\Index{texBundleRelation}%Л%232
   {лифт соответствия}%
   {lift of correspondence}%
\Index{texRefernceFrame}%Л%117
   {локальная система отсчёта}%
   {local reference frame}%
\Index{texBundle}%Л%363
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index{texBundle}%Л%362
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index{texTstarRepresentation}%М%343
   {малая группа}%
   {little group}%
\Index{texDrcMorphism}%М%118
   {матрица \drc линейного отображения}%
   {matrix of drc linear map}%
\Index{texGeomObject}%М%119
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index{texDrcBasis}%М%120
   {многообразие базисов}%
   {}%
\SubIndex{texDrcBasis}%24%
   {\drc векторного пространства}%
   {basis manifold of vector space}%
\SubIndex{texTypeBasis}%25%
   {аффинного пространства}%
   {Basis Manifold, Affine Space}%
\SubIndex{texTypeBasis}%26%
   {евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\SubIndex{texTypeBasis}%27%
   {центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texBasis}%М%276
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index{texBasis}%М%268
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index{texBasis}%М%282
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index{texBasis}%М%280
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texDrcReferenceFrame}%М%123
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index{texFiberedMorphism}%М%355
   {морфизм \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {morphism of representations of fibered F algebra}%
\Index{texTstarMorphism}%М%298
   {морфизм \Ts представлений $\mathfrak{F}$\Hyph алгебры}%
   {morphism of representations of F algebra}%
\Index{texTstarMorphism}%М%300
   {морфизм \Ts представлений $\mathfrak{F}$\Hyph алгебры в $\mathfrak{H}$\Hyph алгебре}%
   {morphism of representations of F algebra in H algebra}%
\Index{texTstarMorphism}%М%307
   {морфизм \Ts представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index{texFiberedMorphism}%М%356
   {морфизм расслоенных \Ts представлений из $\mathcal{F}$ в $\mathcal{G}$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index{texVectorSpace}%Н%124
   {невырожденная система \drc линейных уравнений}%
   {nonsingular system of linear equations}%
\Index{texRepresentation}%Н%241
   {невырожденное \Ts преобразование}%
   {nonsingular transformation}%
\Index{texRefernceFrame}%Н%125
   {неголономная координата}%
   {anholonomic coordinate}%
\Index{texRefernceFrame}%Н%126
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index{texRefernceFrame}%Н%127
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index{texRefernceFrame}%Н%110
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index{texGeomObject}%Н%128
   {неметричность}%
   {nonmetricity}%
\Index{texBundleRelation}%Н%339
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index{texCalculus}%Н%97
   {норма на \drc векторном пространстве}%
   {norm on drc vector space}%
\Index{texCalculus}%Н%100
   {норма на теле}%
   {absolute value on skew field}%
\Index{texCalculus}%Н%102
   {нормированное тело}%
   {valued skew field}%
\Index{texCalculus}%Н%104
   {нормированным \drc векторное пространство}%
   {normed drc vector space}%
\SetIndexSpace%
\Index{texBundleRelation}%О%121
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index{texBundleRelation}%О%115
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index{texBiring}%О%129
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index{texRefernceFrame}%О%130
   {объект неголономности}%
   {anholonomity object}%
\Index{texTstarRepresentation}%О%131
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texRepresentation}%О%259
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texFiberedGroup}%О%132
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index{texTstarMorphism}%О%303
   {однотранзитивное представление алгебры $A$}%
   {single transitive representation of algebra}%
\Index{texRepresentation}%О%258
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index{texFiberedAlgebra}%О%323
   {однотранзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {single transitive representation of fibered F-algebra}%
\Index{texFiberedAlgebra}%О%133
   {операция на расслоении}%
   {operation on bundle}%
\Index{texBiring}%О%134
   {определитель матрицы}%
   {determinant}%
\Index{texTstarRepresentation}%О%135
   {орбита \Ts представления группы}%
   {orbit of representation of group}%
\Index{texRepresentation}%О%253
   {орбита представления группы}%
   {orbit of representation of group}%
\Index{texFiberedGroup}%О%136
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index{texBasis}%О%281
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index{texTidal}%О%137
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index{texDrcReferenceFrame}%О%138
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\SetIndexSpace%
\Index{texGeomObject}%П%139
   {параллелограмм}%
   {parallelogram}%
\Index{texTstarRepresentation}%П%140
   {парные представления группы}%
   {twin representations of group}%
\Index{texFiberedGroup}%П%319
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index{texLinearMap}%П%320
   {парные представления тела}%
   {twin representations of skew field}%
\Index{texDrcBasis}%П%141
   {пассивное \Ts представление}%
   {passive representation}%
\Index{texBasis}%П%273
   {пассивное представление}%
   {passive representation}%
\Index{texBasis}%П%272
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index{texNewton}%П%142
   {первый закон Ньютона}%
   {First Newton law}%
\Index{texAffine}%П%143
   {перенос Картана}%
   {Cartan transport}%
\Index{texAffine}%П%144
   {перенос Френе}%
   {Frenet transport}%
\Index{texBundle}%П%220
   {подрасслоение}%
   {subbundle}%
\Index{texPolyvector}%П%358
   {поливектор}%
   {polyvector}%
\Index{texNewton}%П%146
   {потенциальная энергия}%
   {potential energy}%
\Index{texVectorSpace}%П%149
   {правое векторное пространство}%
   {right vector space}%
\Index{texLie}%П%151
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index{texRepresentation}%П%248
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation}%
\Index{texRepresentation}%П%250
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation}%
\Index{texTstarMorphism}%П%304
   {правостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {right-side representation of algebra}%
\Index{texRepresentation}%П%245
   {правостороннее представление группы}%
   {right-side representation of group}%
\Index{texFiberedAlgebra}%П%324
   {правостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {right-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%П%242
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texRepresentation}%П%243
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texLie}%П%153
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index{texVectorSpace}%П%215
   {правый модуль}%
   {right module}%
\Index{texTstarRepresentation}%П%158
   {правый сдвиг}%
   {right shift}%
\Index{texRepresentation}%П%252
   {правый сдвиг на группе}%
   {right shift, group}%
\Index{texBundleRelation}%П%342
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index{texBundleRelation}%П%335
   {предел фильтра}%
   {limit of filter}%
\Index{texBundleRelation}%П%334
   {предельное множество фильтра}%
   {limit set of filter}%
\Index{texBasis}%П%292
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texDrcBasis}%П%159
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texTstarRepresentation}%П%161
   {представление группы}%
   {}%
\SubIndex{texDrcBasis}%38%
   {\drc линейное \sT}%
   {linear representation of group}%
\SubIndex{texDrcBasis}%39%
   {\rcd}%
   {rcd linear representation of group}%
\SubIndex{texTstarRepresentation}%40%
   {\sT}%
   {starT representation of group}%
\SubIndex{texTstarRepresentation}%41%
   {\Ts}%
   {Tstar representation of group}%
\SubIndex{texTstarRepresentation}%42%
   {ковариантное \Ts}%
   {Tstar covariant representation of group}%
\SubIndex{texTstarRepresentation}%43%
   {контравариантное \Ts}%
   {Tstar contravariant representation of group}%
\SubIndex{texTstarRepresentation}%44%
   {эффективное}%
   {effective representation of group}%
\Index{texRepresentation}%П%246
   {представление группы}%
   {representation of group}%
\Index{texRefernceFrame}%П%165
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index{texTstarMorphism}%П%313
   {преобразование множества}%
   {transformation of set}%
\Index{texDrcBasis}%П%166
   {преобразование на многообразии базисов}%
   {}%
\SubIndex{texDrcBasis}%62%
   {активное}%
   {active transformation, vector space}%
\SubIndex{texTypeBasis}%63%
   {аффинное}%
   {affine transformation}%
\SubIndex{texTypeBasis}%64%
   {движение}%
   {movement transformation}%
\SubIndex{texTypeBasis}%65%
   {квазиаффинное}%
   {quasi affine transformation}%
\SubIndex{texTypeBasis}%66%
   {квазидвижение}%
   {quasi movement}%
\SubIndex{texDrcBasis}%67%
   {пассивное}%
   {passive transformation, vector space}%
\Index{texFiberedAlgebra}%П%329
   {преобразование расслоения}%
   {transformation of bundle}%
\Index{texCartesian}%П%221
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index{texCartesian}%П%222
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index{texBundleRelation,texBundleRelation}%П%225
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index{texBundleRelation}%П%226
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index{texBiring}%П%168
   {приводимое бикольцо}%
   {reducible biring}%
\Index{texBiring}%П%169
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index{texBiring}%П%170
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index{texDrcBasis}%П%171
   {принцип инвариантности}%
   {invariance principle}%
\Index{texBasis}%П%296
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index{texBundleRelation}%П%235
   {продолжение соответствия}%
   {extension of correspondence}%
\Index{texBundle}%П%354
   {проекция расслоения $\mathcal{E}$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index{texDrcBasis}%П%173
   {произведение геометрического объекта и константы}%
   {product of geometrical object and constant}%
\Index{texBasis}%П%295
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometrical object and constant, vector space}%
\Index{texTstarMorphism}%П%299
   {произведение морфизмов \Ts представлений $\mathfrak{F}$\Hyph алгебры}%
   {product of morphisms of representations of F algebra}%
\Index{texBundleRelation}%П%154
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index{texBundleRelation}%П%188
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\SubIndex{texVectorSpace}%74%
   {\drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\SubIndex{texVectorSpace}%75%
   {\rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index{texAffine}%П%174
   {производная Картана}%
   {Cartan derivative}%
\Index{texDiffProperty}%П%175
   {производная Ли}%
   {Lie derivative}%
\SubIndex{texDiffProperty}%72%
   {метрики}%
   {Lie derivative of metric}%
\SubIndex{texDiffProperty}%73%
   {связности}%
   {Lie derivative of connection}%
\Index{texPolyvector}%П%359
   {простой поливектор}%
   {simple polyvector}%
\Index{texTstarRepresentation}%П%352
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index{texCartesian}%П%333
   {пространство отображений}%
   {mapping space}%
\Index{texBundleRelation}%П%236
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index{texLieRepresentation}%П%177
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index{texTstarRepresentation}%П%178
   {прямое произведение \Ts представлений группы}%
   {direct product of representations of group}%
\Index{texRepresentation}%П%254
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index{texFiberedGroup}%П%179
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index{texRefernceFrame}%П%182
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index{texVectorSpace}%Р%183
   {размерность \drc векторного пространства}%
   {dimension of vector space}%
\Index{texFiberedMorphism}%Р%350
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index{texFiberedMorphism}%Р%349
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index{texFiberedAlgebra}%Р%184
   {расслоенная $\mathfrak{F}$\Hyph алгебра}%
   {fibered F-algebra}%
\Index{texFiberedAlgebra}%Р%186
   {расслоенная $\mathfrak{F}$\Hyph подалгебра}%
   {fibered F-subalgebra}%
\Index{texFiberedAlgebra}%Р%185
   {расслоенная группа}%
   {fibered group}%
\Index{texFiberedMorphism}%Р%347
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index{texFiberedMorphism}%Р%346
   {расслоенная малая группа}%
   {fibered little group}%
\Index{texBundleRelation}%Р%145
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index{texBundleRelation}%Р%237
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index{texBundleRelation}%Р%238
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index{texFiberedAlgebra}%Р%187
   {расслоенное кольцо}%
   {fibered ring}%
\Index{texBundle}%Р%219
   {расслоенное подмножество}%
   {fibered subset}%
\Index{texBundleRelation}%Р%224
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index{texBundleRelation}%Р%330
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index{texBundleRelation}%Р%223
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index{texFiberedMorphism}%Р%337
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index{texBundle}%Р%353
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Index{texFiberedMorphism}%Р%338
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index{texBundleRelation}%Р%157
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\SetIndexSpace%
\Index{texTstarRepresentation}%С%345
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index{texFiberedMorphism}%С%348
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index{texAffine}%С%189
   {связность Картана}%
   {Cartan connection}%
\Index{texAffine}%С%190
   {символ Картана}%
   {Cartan symbol}%
\Index{texBiring}%С%191
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index{texBundleRelation}%С%148
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index{texGenRelativity}%С%192
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index{texVectorSpace}%С%193
   {система \drc линейных уравнений}%
   {system of linear equations}%
\Index{texRefernceFrame}%С%194
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index{texNewton}%С%196
   {скалярный потенциал}%
   {scalar potential}%
\Index{texTidal}%С%197
   {скорость отклонения}%
   {speed of deviation}%
\Index{texBundleRelation}%С%297
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index{texBundleRelation}%С%340
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index{texBiring}%С%198
   {стандартное представление матрицы}%
   {Standard representation}%
\Index{texDrcBasis}%С%199
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBasis}%С%269
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBundleRelation}%С%234
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index{texLinearMap}%С%200
   {сумма \drc линейных отображений}%
   {sum of drc linear maps, drc vector spaces}%
\Index{texDrcBasis}%С%201
   {сумма геометрических объектов}%
   {sum of geometrical objects}%
\Index{texBasis}%С%294
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometrical objects, vector space}%
\SetIndexSpace%
\Index{texGeomObject}%Т%95
   {тензор кручения}%
   {torsion tensor}%
\Index{texNewton}%Т%202
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index{texLie}%Т%203
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index{texVectorSpace}%Т%204
   {тип векторного пространства}%
   {vector space type}%
\Index{texCalculus}%Т%152
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index{texCalculus}%Т%33
   {топологическое тело}%
   {topological skew field}%
\Index{texBundleRelation}%Т%147
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index{texTstarMorphism}%Т%305
   {транзитивное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index{texRepresentation}%Т%257
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index{texFiberedAlgebra}%Т%325
   {транзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {transitive representation of fibered F-algebra}%
\SetIndexSpace%
\Index{texDiffProperty}%У%206
   {уравнение Килинга}%
   {Killing equation}%
\Index{texDiffProperty}%У%207
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index{texBiring}%У%208
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index{texFiberedMorphism}%Ф%336
   {фактор расслоение}%
   {quotient bundle}%
\Index{texBundleRelation}%Ф%341
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index{texGeomObject}%Ф%239
   {форма кручение}%
   {torsion form}%
\Index{texCalculus}%Ф%150
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index{texCalculus}%Ф%68
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index{texBasis}%Ц%279
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index{texCalculus}%Ч%106
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, skew field}%
\Index{texCalculus}%Ч%107
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, drc vector space}%
\SetIndexSpace%
\Index{texAffine}%Э%209
   {экстремальная кривая}%
   {extreme line}%
\Index{texTstarMorphism}%Э%306
   {эффективное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index{texRepresentation}%Э%256
   {эффективное представление группы}%
   {effective representation of group}%
\Index{texFiberedAlgebra}%Э%326
   {эффективное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {effective representation of fibered F-algebra}%
\Index{texFiberedGroup}%Э%315
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index{texVectorSpace}%Э%210
   {эффективное представление тела}%
   {effective representation of skew field}%
\SetIndexSpace%
\Index{texTstarRepresentation}%Я%211
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of representation of group}%
\Index{texRepresentation}%Я%255
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index{texFiberedGroup}%Я%212
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%

\CloseIndex


==> Intro.Russian.tex <==
%auto-ignore
\def\texIntro{}

\ifx\PrintBook\Defined
				\chapter{Введение}
			\section{Об этой книге}
			\label{section: About This Book}

Иногда очень трудно дать имя книге, которую ты хочешь написать.
Даже если тв писал эту книгу всю жизнь. А может быть по этой причине.
Путь не завершён. Но я чувствую, настало время поделиться с другими
моими открытиями. Только будущее покажет, какая часть этого исследования
будет полезна.
Эта книга начинается с изучения геометрического объекта, переходит к
системе отсчёта в физике, затем внезапно меняет направление
к изучению метрико\hyph аффинного многообразия.

С тех пор, как Эйнштейн создал общую теорию относительности,
тесная связь между геометрией
и физикой стала реальностью. В тоже время квантовая механика вводит новые концепции, которые
противоречат традиции, установленной на протяжении столетий.
Это означает, что нам нужны новые геометрические концепции, которые станут частью
языка квантовой механики.
Это причина, чтобы вернуться к истокам.

Вся моя жизнь была посвящена решению одной из самых больших
загадок, которую я встретил в начале моей жизни. Когда я познакомился с
общей теорией относительности и квантовой механикой, я почувствовал, что язык
квантовой механики не адекватен явлениям, которые она наблюдает.
Я имею в виду геометрию.

Я посвятил главу \ref{chapter: Space and Time in Physics}
небольшому сочинению, написанному мной, когда я был молод.\footnote{К сожалению,
некоторые ссылки потеряны. Я буду признателен, если кто-то узнает
\label{footnote: Space and Time in Physics}
знакомый текст и даст мне знать точную ссылку.}
\fi

\ifx\texPrefaceRefernceFrame\Defined
\section{Геометрический объект и принцип инвариантности}

\ifx\PrintBook\Defined
Разделы \ref{section: Basis in Vector Space}
и \ref{section: Geometrical Object of Vector Space}
были написаны под большим влиянием книги \citeBib{Rashevsky}.
Изучение однородного пространтва группы симметрии векторного пространства
ведёт нас к определению базиса этого пространства. Многообразие базисов - это множество
базисов изучаемого векторного пространства и является примером однородного пространтва.
Как показано в \citeBib{Rashevsky}, это даёт возможность определить
концепцию инвариантности и геометрического объекта.

Мы определяем два типа преобразований многообразия базисов:
активные и пасивные преобразования. Различие между ними состоит в том,
что пасивное преобразование может быть выражено как преобразование
исходного пространства.

Это определение может быть распространено на произвольное многообразие. Однако в
этом случае мы обобщаем определение базиса и вводим систему
отсчёта. В случае пространтва событий общей теорией относительности это приводит нас к
естественному определению системы отсчёта и преобразованию Лоренца.
Система отсчёта в пространтве событий - это непрерывное поле ортонормальных базисов.
\fi

Принцип инвариантности, рассмотренный в \citeBib{0412.391},
ограничен векторными пространствами и применим только
в рамках специальной теории относительности. Наша задача
описать конструкции, которые позволяют распространить
принцип инвариантности на общую теорию относительности.

Измерение пространственного интервала и временных отрезков
является одной из важных задач общей теории относительности.
Это физический процесс, который позволяет изучать
геометрию в определённой области пространства времени.
С точки зрения геометрии, наблюдатель пользуется ортогональным базисом в касательной
плоскости как своим измерительным инструментом,
так как ортогональный базис приводит к простейшей локальной геометрии.
Двигаясь от точки к точке, наблюдатель переносит с собой свой измерительный прибор.

Понятие геометрического объекта тесно связано с
физическими величинами, измеряемыми в пространстве времени.
Принцип инвариантности позволяет выразить физические законы
независимо от выбора базиса. С другой стороны, если мы хотим
проверить полученное соотношение в опыте, мы должны зафиксировать
измерительный прибор. В нашем случае - это базис. Выбрав
базис, мы можем определить координаты геометрического
объекта, соответствующего изучаемой физической величине.
Следовательно мы можем определить измеряемое значение.

Каждая система отсчёта снабжена неголономными координатами.
Например, синхронизация системы отсчёта - это неголономная координата времени.
Простые расчёты показывают как синхронизация влияет на измерение времени в
окрестности Земли.
Измерение эффекта Допплера от звезды, вращающейся вокруг чёрной дыры, помогает
определить массу чёрной дыры.

Разделы \ref{section: Time Delay in Central Body Gravitational Field}
и \ref{section: Lorentz Transformation in Orbital Direction}
показывают важность расчётов в ортогональном
базисе. Координаты, которыми мы пользуемся в пространстве событий,
- это просто метки
и расчёты, которые мы выполняем в координатах могут оказаться
не надёжными. Например, в статьях \citeBib{Tartaglia,Tomozawa}
авторы определяют координатную скорость света. Это ведёт к
неверному ответу и в результате этого к
различию скорости света в разных направлениях.
\fi

\ifx\texPrefaceTidal\Defined
	\def\texPrefaceTidalOrPrefaceRefernceFrame{}
\fi
\ifx\texPrefaceRefernceFrame\Defined
	\def\texPrefaceTidalOrPrefaceRefernceFrame{}
\fi
\ifx\texPrefaceTidalOrPrefaceRefernceFrame\Defined
Моё внимание привлекла статья \citeBib{Ranada}. Чтобы объяснить аномальное ускорение Pioneer 10
и Pioneer 11 (\citeBib{Anderson02}), Антонио Ранада привлекает старую точку зрения Эйнштейна
о природе гравитационного поля и используют идею Эйнштейна о переменной скорости света.
Когда Эйнштейн начал изучать гравитационное поле, он старался
сохранить геометрию Минковского и, следовательно, предполагал, что масштаб
пространства и времени не меняются. В результате он был вынужден принять гипотезу, что скорость света может
меняться в гравитационном поле. Когда Гроссман познакомил Эйнштейна с римановой геометрией, Эйнштейн
понял, что начальная гипотеза была ошибочна и риманова геометрия лучше решит его задачу.
Эйнштейн никогда
не возвращался к идее о переменной скорости
света.

Действительно, три значения: масштаб пространства и времени и скорость света являются связанными в современной
теории и мы не можем изменить одну величину без изменения другой.
Присутствие гравитационного поля меняет это соотношение. Мы имеем два выбора. Мы сохраняем
исходно заданную геометрию (здесь, геометрию Минковского) и мы согласны, что скорость света
меняется от точки к точке. Риманова геометрия предлагает нам другой выбор. Геометрия становится
результатом измерения и измерительный инструмент может меняться от точки к точке. В этом случае
мы можем сохранить скорость света постоянной. Геометрия становится фоном, который зависит от
физических процессов. Физические законы становятся независимыми от фона.
\fi

\ifx\texPrefaceRefernceFrame\Defined
Некоторые статьи посвящены теории переменной скорости света
\citeBib{Magueijo,Bassett}. Их теория основана на идее, что метрический тензор
может быть инвариантен относительно преобразования подобия. Эта идея не нова.
Как только Эйнштейн опубликовал общую теории относительности,
Вейль предложил свою идею сделать теорию инвариантной относительно
конформного преобразования. Тем не менее, Эйнштейн возражал
этой идее, так как она разрушала зависимость между расстоянием
и собственным временем. Мы можем найти детальный анализ в \citeBib{Straumann}.

Мы имеем тесную связь между скоростью света
и единицами длины и времени в специальной и общей теории относительности.
Когда мы развиваем новую теорию и обнаруживаем, что скорость света меняется,
мы должны спросить себя о причине. Сделали ли мы аккуратное измерение?
Имеем ли мы альтернативный путь для обмена информацией и синхронизации
системы отсчёта? Меняются ли преобразования между системами отсчёта
и образуют ли они группу?

В некоторых моделях фотон может иметь небольшую массу покоя \citeBib{Lammerzahl}.
В этом случае скорость света отлична от максимальной скорости и может
зависеть от направления. Недавний эксперимент \citeBib{Muller}
наложил ограничения на параметры этих моделей.
\fi

\ifx\texPrefaceTorsion\Defined
\section{Тензор кручения в общей теории относительности}

Тесная связь между метрическим тензором и связностью является
основой римановой геометрии.
В то же время, связность и метрика, как любой геометрический объект, являются объектом измерения.
Когда Гильберт выводил уравнение Эйнштейна, он определил лагранжиан, в котором
метрический тензор и связность независимы.
Позже Гильберт обнаружил, что связность
симметрична, и нашёл зависимость между связностью и метрическим тензором. Одна из причин
этого - простота лагранжиана.

\ifx\PrintBook\Defined
Глава \ref{chapter: General Relativistic Field Equations}
формально завершает книгу, хотя исторически она отображает
исследование, с которого начался определённый этап моей жизни.
В основу уравнений, выведенных в этой главе, было положено
непосредственное объединение двух лагранжианов: гравитационного
и квантового полей.
Уравнения
\eqref{eq: Field}, \eqref{eq: Einstein},
\eqref{eq: Cartan} и
\eqref{eq: Maxwell} имеют очень сложный вид.
Они нелинейны по связности.
Но любая попытка решить систему этих уравнений приводит к тому,
что эта системв распадается на уравнение Эйнштейна и
уравнение поля, которые независимы.
Повидимому неудача изначально заложена в самом подходе к проблеме.
Последующее развитие физики показало, что объединение общей теории
относительности и квантовой механики требует более мощных методов.
Основные направления на сегодняшний день можно разделить на теорию
струн и петлевую теорию гравитации.

Однако несмотря на неудачу, анализ полученных уравнений очень важен.
\fi

Анализ квантовой теории поля показывает,что либо
симметрия связности, либо зависимость связности и метрики могут быть нарушены, 
поскольку неизбежны ошибки измерения.
Это допущение приводит к метрико\hyph аффинному многообразию,
которое является пространством с кручением и ненулевой ковариантной производной
метрического тензора (раздел \ref{section: Metric-affine Manifold}).
Независимость метрического тензора и связности позволяет нам видеть, какие
объекты ответственны за различные
явления в геометрии и, следовательно, в физике.
Даже несмотря на то, что мы не доказали эмпирически
существование кручения и неметричности, мы видим здесь очень интересную геометрию.

Метрико\hyph аффинное многообразие появляется в разных физических приложениях.
Очень важно понять какова геометрия этого пространства,
как кручение может влиять на физические процессы.
Именно поэтому небольшая группа физиков продолжает изучать теорию
гравитации с кручением
\citeBib{Mielke,Obukhov,Sardanashvily,Gauge,Neeman}.

В частности, мы имеем два различных определения геодезической в римановом многообразие.
Мы можем рассматривать геодезическую либо как кривую экстремальной длины
(соответствующую кривую мы называем экстремальной),
либо как кривую, вдоль которой касательный вектор переносится параллельно, оставаясь
касательным к кривой
(соответствующую кривую мы называем автопараллельной).
Неметричность приводит к тому, что параллельный
перенос не сохраняет длину вектора и угол между
векторами. Это приводит к различию между
определениями автопараллельной и экстремальной кривых (\citeBib{torsion} и
раздел \ref{section: Line with extreme length})
и к изменению в выражении переноса Френе.
Изменение геометрии влияет на второй закон Ньютона, который
мы изучаем в разделе \ref{section: Newton Laws: Scalar Potential}.
Я показываю в теоремах \ref{theorem: LengthTangentVector} и \ref{theorem: First Newton law},
что свободно падающая частица предпочитает экстремальную кривую, перенося
свой импульс вдоль траектории без изменения.

Форма второго закона Ньютона зависит от выбора формы потенциала.
В случае скалярного потенциала
второй закон Ньютона сохраняет соотношение между силой, массой и ускорением.
В случае векторного потенциала
анализ движения в гравитационном поле показывает, что тензор напряжённости поля
зависит от производной метрического тензора.

Неметричность значительно изменяет закон движения в пространстве
времени ортогонального базиса.
Однакко изучение параллельного переноса в пространстве с неметричностью позволяет нам
ввести перенос Картана и введение связности, совместимой с метрическим тензором
(раздел \ref{section: Cartan Transport}). Перенос Картана
сохраняет базис ортонормальным и это делает его важным инструментом
в динамике (раздел \ref{section: Newton Laws: Scalar Potential}),
так как наблюдатель использует ортонормальный базис как инструмент измерения.
Динамика частицы основана на переносе Картана.
Тогда появляется вопрос.
Мы можем изменить связность как мы показали в разделе \ref{section: Cartan Transport}.
%or мы can change the metric tensor as is shown
%in  such way that the parallel transport conserves
%the metric tensor\footnote{I am not agree with conclussion in paper \cite{Hehl},
%however this paper shows way how to find the metric tensor compatible with connection}.
Почему мы должны изучать многообразия с произвольной связностью и метрическим тензором?
Изучение метрико\hyph аффинного многообразия показывает, почему всё
работает хорощо в римановом многообразии и что меняется в общем случае.
К какого рода различные физические явления
являются следствием различных связностей?
Физические ограничения, которые появляются в модели, могут вести к появлению неметричности
\citeBib{Gauge,Megged,gr-qc-9604027}.
Так как перенос Картана - естественный механизм сохранения ортогональности,
мы ожидаем, что мы будем интерпретировать отклонение
пробной частицы от экстремальной кривой как
результат силы, внешней по отношению к этой частице\footnote{Например,
если мы распространим определение \eqref{eq: potential force} силы
на общий случай \eqref{eq: Newton}, мы можем интерпретировать отклонение заряжённой
частицы в электромагнитном поле как результат силы
\[\ F^j=\frac e {cu^0} g^{ij} F_{li} u^l\]
Аналогично, мы можем интерпретировать отклонение автопараллельной кривой как силу
\[F^i=-\frac {m c} {u^0} \Gamma(C)^i_{kl}u^ku^l\]
Я напоминаю, что символ Картана - тензор}.
В этом случае различие между двумя типами переноса
становится измеримым и осмысленным. В противном случае другой тип
переноса и неметричность не наблюдаемы и мы можем пользоваться
только переносом, совместимым с метрикой.

Я вижу ещё одну возможность. Как следует из статьи \citeBib{Megged},
кручение может зависеть от квантовых свойств материи.
Тем не менее, кручение является частью связности. Следовательно, связность может
также зависеть от квантовых свойств материи. Это может привести к нарушению
переноса Картана. Однако эта возможность требует дополнительного иследования.

Кручение и неметричность имеют интегральные эффекты.
Они могут быть малыми, но измеримыми. Мы можем наблюдать эти эффекты не только в сильных
полях, подобных чёрной дыре или большому взрыву, но также в обычных условиях.
Изучение геометрии и линамики точечной частицы даёт нам возможность
проверить эту точку зрения.
Есть смысл проверить эту теорию в условиях, когда спин квантового поля накоплен.
Мы можем проверить отклонение от второго закона Ньютона либо измерить кручение,
наблюдая движение двух различных ыастиц.

Чтобы проверить, имеет ли пространство время кручение, мы
можем проверить возможность построить параллелограмм в пространстве времени. 
Мы можем взять две частицы или два фотона,
которые начинают своё движение из одной и той же точки
и, пользуясь зеркалом, заставить их двигаться вдоль противоположных
сторон параллелограмма.
Мы можем начать этот эксперимент, когда квантового поля нет, и затем повторить
эксперимент в присутствии квантового поля.
Если частицы встретятся в одном и том же месте или мы имеем одинаковую
интерференцию, то мы имеем
кручение равное $0$ в этой среде.
В частности, кручение может действовать на поведение виртуальных частиц.

Чтобы проверить, имеет ли пространство время неметричность, мы
можем измерить отклонение экстремальной кривой
от автопараллельной либо
отклонение единичного вектора скорости от его параллельного переноса.
\fi

\ifx\PrintBook\Defined
\section{Симметрия}

The torsion leads to a change in the Killing equation. Мы also need to add a similar equation
for the connection.

Ассиметрия связности возникает не только за счёт кручения. Изучение теории
геометрического объекта в векторном пространстве приводит к её естественному
обобщению: теории системы отсчёта в пространстве событий. Система отсчёта
является мощнейшим измерительным инструментом в общей теории относительности.
\fi

\ifx\texPrefaceTidal\Defined

\section{Приливное ускорение}

Наблюдения в Солнечной системе и вне очень важны. Они дают нам возможность
видеть, где общая теория относительности права и найти её ограничения.
Очень важно быть осторожным с такими наблюдениями.
NASA выполнило очень интересные наблюдения Pioneer 10 и Pioneer 11
и выполнило сложные расчёты их ускорения. Однако, возникает один интересный
вопрос: какого типа ускорения мы меряли?

Pioneer 10 и Pioneer 11 совершают свободное движение в солнечной системе.
Следовательно, они движутся вдоль своей траектории без ускорения.
Однако, хорошо известно, что два тела, двигаясь вдоль близких геодезических, имеют относительное
ускорение, которое называется приливным ускорением. Приливное ускорение
в общей теории относительности имеет вид
	\begin{equation}
	\label{eq: Tidal acceleration}
\frac{D^2\delta x^k}{ds^2}
=R^k_{lnk}\delta x^kv^nv^l
	\end{equation}
где $v^l$ - скорость тела $1$ и $\delta x^k$ - отклонение геодезической тела $2$
от геодезической тела $1$. Мы видим из этого выражения, что приливное ускорение
зависит от движения тела $1$ и как траектория тела $2$ отклоняется от траектории тела $1$.
Но это значит, что даже для двух тел, которые находятся на одном и том же
расстоянии от центрального тела, мы можем измерить
разное ускорение относительно наблюдателя.

Раздел \ref{section: Tidal Equation} посвящён решению задачи,
какие изменения испытывает приливная сила на метрико\hyph аффинном многообразии.

Возникает вопрос: можем ли мы использовать уравнение \eqref{eq: deviation_extreme},
чтобы измерить кручение? Мы получим приливное ускорение из прямых измерений. Существует
метод измерять кривизну (см. например \citeBib{Wheeler}). Однако, даже
если мы знаем ускорение и кривизну, мы по\Hyph прежнему имеем дифференциальное уравнение,
чтобы найти кручение. Однако, этот путь может дать прямой ответ на вопрос
существует ли кручение.

Отклонение от приливного ускорения \eqref{eq: Tidal acceleration},
предсказанного общей теорией относительности может иметь различные причины.
Однако мы можем найти ответ, комбинируя разные методы измерения.
\fi


==> Newton.Russian.tex <==
%auto-ignore
\def\texNewton{}
\ifx\PrintBook\Defined
				\chapter{Метрико-аффинная гравитация}
\fi

\section{Закон Ньютона: скалярный потенциал}
\label{section: Newton Laws: Scalar Potential}

Знание динамики точечной частицы важно для нас,
так как мы можем изучать как частица взаимодействует с внешними полями,
так же как свойства самой частицы.

Чтобы изучить движение точечной частицы, мы можем использовать потенциал определённых полей.
Потенциал может быть скалярным или векторным.

В случае скалярного потенциала мы положим, что точечная частица
имеет массу покоя $m$ и мы пользуемся функцией Лагранжа в следующем виде
\[L = - m c ds - U dx^0\]о
где $U$ - \AddIndex{скалярный потенциал}{scalar potential}
или \AddIndex{потенциальная энергия}{potential energy}.

		\begin{theorem}
		\label{theorem: First Newton law}
(\AddIndex{Первый закон Ньютона}{First Newton law})
Если $U = 0$ (следовательно, мы рассматриваем свободное движение),
то тело выбирает траекторию с экстремальной длиной.
		\end{theorem}

		\begin{theorem}
(\AddIndex{Второй закон Ньютона}{Second Newton law})
Траекторию точечной частицы удовлетворяет дифференциальному уравнению
	\begin{equation}
\frac {\overbrace{D}u^l} {ds} =
\frac {u^0} {m c} F^l
	\label{eq: Newton}
	\end{equation}
\[u^j = \frac {dx^l} {ds}\]
где мы определяем силу
	\begin{equation}
F^l = g^{il} \frac{\partial U}{\partial x^i}
\label{eq: potential force}
	\end{equation}
		\end{theorem}
		\begin{proof}

Пользуясь \eqref{eq: VarLineLength},
мы можем записать вариацию лагранжиана в виде
$$\frac 1 2 m c \left(g_{kl;i} - g_{ik;l}
- g_{il;k}\right) u^k u^j ds
- m c g_{ij} Du^j
+ \frac {\partial U} {\partial x^i} dx^0 = 0$$
Отсюда следует утверждение теоремы.
		\end{proof}

			\section{Закон Ньютона: векторный потенциал}
В разделе \ref{section: Newton Laws: Scalar Potential}
мы изучили динамику скалярного потенциала.
Однако в электродинамике мы рассматриваем \AddIndex{векторный потенциал}
{vector potential} $A^k$.
В этом случае действие имеет вид
\[
S = \int^{t_2}_{t_1} \left( - m c ds - \frac e c A_l dx^l \right)
\]
\[
A_c = g_{cd} A^d
\]

		\begin{theorem}
Траектория частицы, движущейся в векторном поле, удовлетворяет дифференциальному уравнению
\[
\frac {\overbrace{D}u^j} {ds} =
\frac e {m c^2} g^{ij} F_{li} u^l
\]
\[u^j = \frac {dx^l} {ds}\]
где мы определяем \AddIndex{тензор напряжённости поля}
{field-strength tensor}
\[F_{dc} = A_{d;c} - A_{c;d} + S^p_{dc} A_p
 = \overbrace{\nabla_c}A_d - \overbrace{\nabla_d}A_c + S^p_{dc} A_p\]
		\end{theorem}
		\begin{proof}

Пользуясь \eqref{eq: VarLineLength}, мы можем записать вариацию действия в виде
%\begin{widetext}
\[
\delta S =\]
\[=\int^{t_2}_{t_1} \left( - m c \left(
\frac 1 2 \left( g_{kj;i}
- g_{ij;k} - g_{ik;j} \right) u^k u^j ds
- g_{ij} D u^j\right) \delta x^i
- \frac e c \left(\delta A_l dx^l + A_l \delta dx^l \right)
\right)
\]
%\end{widetext}
Мы можем оценить второе слагаемое
\[
- \frac e c \left(A_{l,k} dx^l \delta x^k + A_l d\delta x^l \right) =
\]
\[
=- \frac e c \left(A_{l;k} dx^l \delta x^k
+ \Gamma^p_{lk} A_p dx^l \delta x^k
+ A_l d\delta x^l \right) =
\]
%\begin{widetext}
\[
=- \frac e c \left(A_{k;l} dx^l \delta x^k +
\left(A_{l;k} - A_{k;l}\right)dx^l \delta x^k+
S^p_{lk} A_p dx^l \delta x^k + \Gamma^p_{kl} A_p dx^l \delta x^k
+ A_l d\delta x^l \right) =
\]
\[
=- \frac e c \left(DA_k \delta x^k + A_k D\delta x^k +
\left(A_{l;k} - A_{k;l}\right)dx^l \delta x^k
+ S^p_{lk} A_p dx^l \delta x^k \right) =
\]
%\end{widetext}
\[
=- \frac e c \left(\underline{d\left(A_k \delta x^k\right)} +
\left( A_{l;k} - A_{k;l}
+ S^p_{lk} A_p \right) dx^l \delta x^k\right)
\]
Интеграл подчёркнутого слагаемого равен $0$,
так как точки, когда $t = t_1$ и $t = t_2$, фиксированы.
Следовательно,
\[
- m c \left(
\frac 1 2 \left( g_{kj;i}
- g_{ij;k} - g_{ik;j} \right) u^k u^j ds
- g_{ij} D u^j\right)-
\frac e c F_{li} dx^l = 0
\]
Отсюда следует утверждение теоремы.
		\end{proof}

Из этой теоремы следует
зависимость тензора напряжённости поля от производной метрики.
Это изменяет форму уравнения Эйнштейна и импульс гравитацинного поля
появляется в случае векторного поля.

		\begin{theorem}
Тензор напряжённости поля не изменяется, когда векторный потенциал изменяется
согласно правилу
\[A'_j=A_j+\partial_j\Lambda\]
где $\Lambda$ - произвольная функция $x$.
		\end{theorem}
		\begin{proof}
Изменение в тензоре напряжённости поля имеет вид
\[(\partial_d\Lambda){}_{;c} - (\partial_c\Lambda){}_{;d} + S^p_{dc} \partial_p\Lambda =\]
\[\partial_{cd}\Lambda - \Gamma^p_{dc} \partial_p\Lambda
- \partial_{dc}\Lambda+\Gamma^p_{cd} \partial_p\Lambda + S^p_{dc}\partial_p\Lambda =0\]
Это доказывет теорему.
		\end{proof}





==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant definition}%
\Symb{texBiring}%
   {минор}%
   {A from b a}%
\Symb{texBiring}%
   {минор}%
   {A from columns T}%
\Symb{texBiring}%
   {минор}%
   {A from rows S}%
\Symb{texBiring}%
   {минор}%
   {A without column a}%
\Symb{texBiring}%
   {минор}%
   {A without columns T}%
\Symb{texBiring}%
   {минор}%
   {A without row b}%
\Symb{texBiring}%
   {минор}%
   {A without rows S}%
\Symb{texPolymodule}%
   {активное преобразование}%
   {active transformation}%
\Symb{texTypeBasis}%
   {аффинное пространство}%
   {affine space}%
\Symb{texBasis}%
   {аффинное пространство}%
   {An}%
\Symb{texBiring}%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb{texBiring}%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb{texBiring}%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb{texBiring}%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb{texVectorSpace}%
   {\dcr вектор}%
   {dcr vector}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb{texVectorSpace}%
   {\drc вектор}%
   {drc vector}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb{texPolymodule}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texBiring}%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb{texBiring}%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb{texBiring}%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb{texBiring}%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb{texBiring}%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb{texTstarRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texPolyvector}%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb{texFiberedGroup}%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb{texTstarRepresentation}%
   {левый сдвиг}%
   {Tstar shift}%
\Symb{texFiberedGroup}%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb{texRefernceFrame}%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb{texRefernceFrame}%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%
\Symb{texBasis}%
   {многообразие базисов аффинного пространства}%
   {BAn}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства $\mathcal{V}$}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb{texBasis}%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb{texBundle}%
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power of bundle}%
\Symb{texBundle}%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb{texTypeBasis}%
   {многообразие базисов аффинного пространства}%
   {FAn}%
\Symb{texTypeBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb{texTypeBasis}%
   {многообразие базисов евклидова пространства}%
   {FEn}%

\SetIndexSpace%
\Symb{texBasis}%
   {центро-аффинное пространство}%
   {CAn}%
\Symb{texTypeBasis}%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb{texLie}%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb{texLie}%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation, coordinates}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation, coordinates}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство \subs строк}%
   {c rows dcr vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to drc vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to skew field}%
\Symb{texVectorSpace}%
   {\drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Symb{texVectorSpace}%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace D}%
\Symb{texAffine}%
   {производная}%
   {overline D}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, skew field}%
\Symb{texVectorSpace}%
   {\drc векторное пространство \sups строк}%
   {r rows drc vector space}%
\Symb{texTidal}%
   {скорость отклонения}%
   {speed of deviation}%
\Symb{texVectorSpace}%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%
\Symb{texTypeBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texTypeBasis}%
   {базис}%
   {basis}%
\Symb{texBasis}%
   {базис векторного пространства}%
   {Basis e}%
\Symb{texBasis}%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb{texVectorSpace}%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb{texPolymodule}%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb{texCartesian}%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb{texBasis}%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb{texRefernceFrame}%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb{texBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texTypeBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texTypeBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texFiberedAlgebra}%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb{texBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb{texBasis}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texRefernceFrame}%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb{texRefernceFrame}%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb{texBasis}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {координаты базиса в \dcr векторном пространстве \subs строк}%
   {basis coordinates, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {координаты базиса в \drc векторном пространстве \sups строк}%
   {basis coordinates, r rows drc vector space}%
\Symb{texVectorSpace}%
   {базис в \dcr векторном пространстве \subs строк}%
   {basis, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {базис в \drc векторного пространства \sups строк}%
   {basis, r rows drc vector space}%
\Symb{texDiffEq}%
   {центро-аффинный}%
   {Central Affine Basis}%
\Symb{texBundle}%
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Symb{texBundleRelation}%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb{texFiberedAlgebra}%
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb{texCartesian}%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb{texTstarRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%
\Symb{texTypeBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texRefernceFrame}%
   {система отсчёта}%
   {reference frame}%
\Symb{texRefernceFrame}%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb{texPolymodule}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texPolymodule}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb{texFiberedMorphism}%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb{texFiberedMorphism}%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb{texLie}%
   {алгебра Ли группы Ли}%
   {g}%
\Symb{texLie}%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb{texTypeBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texLie}%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb{texBasis}%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb{texTstarRepresentation}%
   {малая группа элемента $x$}%
   {little group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective starT covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective starT covariant representation of group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective Tstar covariant representation of group}%
\Symb{texVectorSpace}%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb{texTstarRepresentation}%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%
\Symb{texBiring}%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb{texLinearMap}%
   {\rcd векторное пространство \drc линейных отображений}%
   {rcd vector space of drc linear maps}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb{texLinearLie}%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%
\Symb{texRepresentation}%
   {левый сдвиг}%
   {left shift}%
\Symb{texDiffProperty}%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb{texDiffProperty}%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb{texBundleRelation}%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb{texBasis}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texRepresentation}%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texTstarMorphism}%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb{texTstarMorphism}%
   {множество \Ts преобразований множества $M$}%
   {set of Tstar transformations}%
\Symb{texTstarRepresentation}%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%
\Symb{texBasis}%
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Symb{texBasis}%
   {геометрический объект}%
   {geometrical object, vector space}%
\Symb{texFiberedGroup}%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of fibered group}%
\Symb{texRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%
\Symb{texBundle}%
   {расслоение}%
   {bundle}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb{texCartesian}%
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%
\Symb{texBasis}%
   {активное преобразование}%
   {active transformation}%
\Symb{texAffine}%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb{texVectorSpace}%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb{texAffine}%
   {кривизна}%
   {GLn curvature_overline}%
\Symb{texVectorSpace}%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb{texRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texRepresentation}%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb{texVectorSpace}%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%
\Symb{texLie}%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%
\Symb{texBasis}%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb{texBasis}%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb{texVectorSpace}%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb{texLinearMap}%
   {($S$, $T$)\hyph бимодуль}%
   {R S bimodule}%
\Symb{texVectorSpace}%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb{texVectorSpace}%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb{texBasis}%
   {векторное пространство}%
   {V}%

\SetIndexSpace%
\Symb{texPolymodule}%
   {геометрический объект в координатном представлении,		определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\Symb{texPolymodule}%
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%

\SetIndexSpace%
\Symb{texTidal}%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb{texRepresentation}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texTstarMorphism}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texBasis}%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb{texBiring}%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb{texAffine}%
   {символ Картана}%
   {Cartan symbol}%
\Symb{texAffine}%
   {связность}%
   {conection overline}%
\Symb{texRefernceFrame}%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb{texAffine}%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb{texBundle}%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%
\Symb{texLie}%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb{texLie}%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, skew field}%
\Symb{texRefernceFrame}%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%

\SetIndexSpace%
\Symb{texLie}%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%
\Symb{texBundle}%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb{texBundle}%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

